New Tools, Programming Models, and System Support for Processing-in-Memory Architectures

Our goal in this dissertation is to provide tools, programming models, and system support for PIM architectures (with a focus on DRAM-based solutions), to ease the adoption of PIM in current and future systems. To this end, we make at least four new major contributions. First, we introduce DAMOV, the first rigorous methodology to characterize memory-related data movement bottlenecks in modern workloads, and the first data movement benchmark suite. Second, we introduce MIMDRAM, a new hardware/software co-designed substrate that addresses the major current programmability and flexibility limitations of the bulk bitwise execution model of processing-using-DRAM (PUD) architectures. MIMDRAM enables the allocation and control of only the needed computing resources inside DRAM for PUD computing. Third, we introduce Proteus, the first hardware framework that addresses the high execution latency of bulk bitwise PUD operations in state-of-the-art PUD architectures by implementing a data-aware runtime engine for PUD. Proteus reduces the latency of PUD operations in three different ways: (i) Proteus concurrently executes independent in-DRAM primitives belong to a single PUD operation across DRAM arrays. (ii) Proteus dynamically reduces the bit-precision (and consequentially the latency and energy consumption) of PUD operations by exploiting narrow values (i.e., values with many leading zeros or ones). (iii) Proteus chooses and uses the most appropriate data representation and arithmetic algorithm implementation for a given PUD instruction transparently to the programmer. Fourth, we introduce DaPPA (data-parallel processing-in-memory architecture), a new programming framework that eases programmability for general-purpose PNM architectures by allowing the programmer to write efficient PIM-friendly code without the need to manage hardware resources explicitly.

==> mainmatter/04_damov/Sections/00_abstract.tex <==
%!TEX root=main_paper.tex %
% these percent signs need to be here!
%
Data movement between the CPU and main memory is a first-order obstacle \geraldorevi{against} improv\geraldorevi{ing} performance, scalability, and energy efficiency in modern systems. Computer systems employ a range of techniques to reduce overheads tied to data movement, spanning from traditional mechanisms (e.g., deep \geraldorevi{multi-level} cache hierarch\geraldorevi{ies}, aggressive hardware prefetcher\geraldorevi{s}) to emerging techniques such as Near-Data Processing (NDP), where some computation is moved close to memory. Prior NDP works investigate the root causes of data movement bottlenecks using different profiling methodologies and tools. However, there is still a lack of understanding about the key metrics that can identify different data movement bottlenecks and their relation to traditional and emerging data movement mitigation mechanisms. Our goal is to methodically identify potential sources of data movement over a broad set of applications \geraldorevi{and to comprehensively compare traditional compute-centric data movement mitigation techniques (e.g., cach\gfiii{ing} and prefetch\gfiii{ing}) to more memory-centric techniques (e.g., NDP), \gfiii{thereby developing a rigorous understanding of} the best techniques \geraldorevii{to mitigate} each source of data movement.}

With this goal in mind, we perform the first large-scale characterization of \geraldorevii{a wide variety} \gfiii{of} \sg{applications, across a wide range of application domains,} to identify fundamental program properties that lead to data movement to/from main memory. We develop the first systematic methodology to classify \gfiii{applications} based on the sources contributing to data movement bottlenecks. From our large-scale characterization \gfiii{of 77K functions across 345 applications}, we select 144 \geraldorevii{functions} to form the first open-source benchmark suite \geraldorevii{(\bench)} for main memory data movement studies. We select a diverse range of \geraldorevii{functions} that (1)~represent different types of data movement bottlenecks, and (2)~come from a wide range of application domains. Using NDP as a case study, we identify new insights about the different data movement bottlenecks and use these insights to determine the most suitable data movement mitigation mechanism for a particular application. \gfii{We open-source DAMOV and the complete source code for our new characterization methodology at~\url{https://github.com/CMU-SAFARI/DAMOV}.}



==> mainmatter/04_damov/Sections/06_related_work.tex <==
\section{Related Work}

\geraldorevi{To our knowledge, this is the first work that methodically characterizes data movement bottlenecks and evaluates the benefits of different data movement mitigation mechanisms, with a focus on Near-Data Processing (NDP), for a broad range of applications. This is also the first work that provides an extensive \gfii{open-source} benchmark suite, with a diverse range of real world applications, tailored to stress different \gfii{memory-related} data movement bottlenecks in a system.}


Many past works investigate how to reduce data movement cost using a range of different compute-centric (e.g., \geraldorevi{prefetchers~\gfvii{\cite{
gonzalez1997speculative,
chen1995effective, 
bera2019dspatch, 
bakhshalipour2018domino, 
fu1992stride, 
ishii2009access, 
hashemi2018learning,
orosa2018avpp,
jog2013orchestrated,
lee2011prefetch,
ebrahimi2009techniques,
srinath2007feedback,
austin1995zero,
ceze2006cava,
kadjo2014b,
kirman2005checkpointed,
cooksey2002stateless,
joseph1997prefetching,
ebrahimi2011prefetch,
ebrahimi2009coordinated,
lee2009improving,
ChangJooLee,charney1995,charneyphd}}, speculative execution~\gfiii{\cite{gonzalez1997speculative, mutlu2003runahead, hashemi2016continuous, mutlu2005techniques,mutlu2006efficient, mutlu2005using}},} value-prediction~\gfiii{\cite{orosa2018avpp, yazdanbakhsh2016rfvp, eickemeyer1993load, endo2017interactions, gonzalez1997speculative, lipasti1996exceeding,lipasti1996value,calder1999selective,wang1997highly,gabbay1996speculative,burtscher1999exploring,fu1998value,goeman2001differential,nakra1999global,sato2002low,sazeides1997predictability,tuck2005multithreaded,tullsen1999storageless,tune2002quantifying}}, data compression~\gfvii{\cite{pekhimenko2012base, 
dusser2009zero, 
yang2000frequent,
alameldeen2004adaptive, 
zhang2000frequent,
pekhimenko2016case,pekhimenko2015toggle, pekhimenkoenergy, pekhimenko2015exploiting, pekhimenko2013linearly,chen2009c,hallnor2005unified,hammerstrom1977information,islam2009zero,arelakis2014sc,ekman2005robust,vijaykumar2015case,gaur2016base}}, approximate computing~\gfiii{\cite{yazdanbakhsh2016rfvp,koppula2019eden,miguel2015doppelganger,oliveira2018employing}}) and memory-centric techniques~\gfvii{\cite{vijaykumar2018case, yazdanbakhsh2016mitigating, joao2012bottleneck, tsai2018rethinking, sembrant2014direct, PEI,lazypim,MEMSYS_MVX,top-pim,acm,New_PIM_2013,kim2017heterogeneous,pugsley2014comparing,boroumand2018google,azarkhish2016memory,nai2017graphpim,gao2016hrl,de2018design,babarinsa2015jafar,tsai2017jenga,tsai2019compress,vijaykumar2018locality,mutlu2020intelligent,mutlu2020intelligentdate}}. \gfii{These works} evaluate the impact of data movement in different systems\geraldorevi{, including} mobile systems~\gfiii{\cite{boroumand2018google, pandiyan2014quantifying, narancic2014evaluating, yan2015characterizing,shingari2015characterization}}, data centers~\gfiii{\cite{kanev_isca2015, ferdman2012clearing, kozyrakis2010server,yasin2014deep, hashemi2018learning, gupta2019architectural,gan2018architectural,ayers2018memory}}, accelerators\gfiii{-}\geraldorevi{based systems}~\gfiii{\cite{boroumand2018google, gupta2019architectural, singh2019napel, murphy2001characterization, cali2020genasm, kim2018grim,alser2020accelerating}}, and \geraldorevi{desktop} computers~\cite{limaye2018workload, bienia2008parsec, corda2019memory}. They use \gfii{very} different profiling frameworks and methodologies to identify the root cause of data movement for a \geraldorevi{small} set of applications. Thus, it is not possible to generalize \gfii{prior works'} findings \gfii{to} other applications \gfii{than the limited set they analyze}.

\geraldorevi{We highlight two of these prior works, \cite{murphy2001characterization} and \cite{boroumand2018google}, since they also} focus on characterizing applications \gfii{for} \gls{NDP} architectures. In \cite{murphy2001characterization}, the authors provide the first work that characterizes workloads for \gls{NDP}. They analyze \geraldorevi{five} applications \geraldorevi{(FFT, ray tracing, method of moments, image understanding, data management)}. The \gls{NDP} organization \cite{murphy2001characterization} targets is similar to \cite{IRAM_Micro_1997}, where \geraldorevi{vector processing compute} units \geraldorevi{are} integrate\geraldorevi{d into} the DDRx memor\geraldorevi{y modules}. Even though \cite{murphy2001characterization} has a similar goal to our work, it understandably does not provide insights \gfii{into} modern data-intensive applications and \gls{NDP} architectures \gfii{as it dates from 2001}. \gfiii{Also, \cite{murphy2001characterization} focus\gfiv{es its} analysis only on a few workloads, whereas we conduct a broader workload analysis starting from 345 applications.} Therefore, a new\gfiii{, more comprehensive and rigorous} analysis methodology of data movement bottlenecks \gfii{in modern workloads and modern NDP systems} is necessary. A more recent work investigates the memory bottlenecks in \gfii{widely-used} \geraldorevi{consumer} workloads \geraldorevi{from Google} and how \gls{NDP} can mitigate \geraldorevi{such bottlenecks} \cite{boroumand2018google}. \geraldorevi{This work} \geraldorevi{focuses its} analysis on a \geraldorevi{small} number of consumer workloads. Our work presents a comprehensive analysis of a much broader set of applications \geraldorevi{(\gfiii{345} different applications, and a total of \gfiii{77K} application functions)}, which allows us to provide \gfii{a general methodology, a comprehensive workload suite, and} general takeaways and guidelines for future \gls{NDP} research. \geraldorevi{\gfii{With our comprehensive analysis, this work is the first to} develop a rigorous methodology to classify applications into six groups, which have different characteristics with respect to how they benefit from NDP \gfii{systems} \gfiii{as well as other data movement bottleneck mitigation techniques}.}




==> mainmatter/04_damov/packages_damov.tex <==
\usepackage{algorithmic}
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{dblfloatfix}   
\usepackage{balance}
\usepackage{xspace}
\usepackage[normalem]{ulem}
\usepackage{fancyhdr}
\usepackage[labelfont=bf, textfont=bf, skip=2pt]{caption}
\usepackage[english]{babel}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{pifont}
\usepackage{footnote}
\usepackage{enumitem}
\usepackage{ltablex}
\usepackage{makecell}
\usepackage{xargs} 
\usepackage{color, colortbl}
\usepackage[multiple]{footmisc}
\usepackage{marginnote}
\usepackage{clipboard}
\usepackage{subcaption}
\usepackage{mathtools}
\usepackage[compact]{titlesec}
\usepackage{wrapfig}
\usepackage{imakeidx}
\usepackage{soul}
\usepackage[keeplastbox]{flushend}
\usepackage[acronym,nonumberlist,nowarn]{glossaries}
    \glsdisablehyper
     \loadglsentries{acronyms}
\usepackage{imakeidx}
\usepackage{graphbox}
\usepackage{cuted,capt-of}
    

==> mainmatter/05_mimdram/packages_mimdram.tex <==
%\usepackage{upmath}

%

\PassOptionsToPackage{hyphens}{url}
\usepackage[bookmarks=true,breaklinks=true,colorlinks,linkcolor=black,citecolor=black,urlcolor=blue]{hyperref}

\usepackage[noadjust]{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage[hyphens]{url}
\usepackage{fancyhdr}
%\usepackage{hyperref}

\usepackage{mathptmx} % This is Times font
\usepackage{setspace}

\usepackage{balance}

\usepackage[acronym,nonumberlist,nowarn]{glossaries}
    \glsdisablehyper
     \loadglsentries{acronyms}
     
\usepackage{footnote}
\usepackage{multicol}
%\usepackage[final]{microtype}
\usepackage{xspace}
\usepackage[normalem]{ulem}
%\usepackage[labelfont=bf, textfont=bf, skip=2pt]{caption}
\usepackage[skip=2pt]{caption}
%\usepackage[english]{babel}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{ltablex}
\usepackage{makecell}
\usepackage[binary-units=true]{siunitx}
\usepackage{xargs} 
\usepackage{color, colortbl}
\usepackage[multiple]{footmisc}
\usepackage{marginnote}
\usepackage{clipboard}
\usepackage{tikz}
\usepackage{subcaption}
\usepackage{mathtools}
\usepackage{longfbox}
\usepackage[compact]{titlesec}
\usepackage{wrapfig}
\usepackage{graphbox}
\usepackage{cuted,capt-of}
\usepackage{todonotes}
\usepackage{soul}
\usepackage[many]{tcolorbox}

%\let\labelindent\relax

\usepackage{enumitem}
\usepackage{xcolor}
\usepackage[us,12hr]{datetime}



\usepackage[en-GB, useregional=numeric]{datetime2}



\usepackage{cleveref}

\crefformat{section}{\S#2#1#3}
\crefformat{subsection}{\S#2#1#3}
\crefformat{subsubsection}{\S#2#1#3}

==> mainmatter/05_mimdram/sections/00_abstract.tex <==
\begin{abstract}

\gfi{\gls{PuD}} is a \gls{PIM} approach that \gf{uses} \om{a} DRAM \omi{array's} massive \om{internal}  parallelism to execute \om{very}-wide \gfcri{(e.g., \gfcrii{16,384--262,144-\omii{bit-}wide}) } \om{data-parallel} operations\gfcri{, in a \gls{SIMD} fashion}. However, DRAM rows' large and rigid granularity \gfcr{limit} the effectiveness and applicability
of \gfi{\gls{PuD}} in \gf{three} ways. 
First, since \gfcrii{applications \omiii{have} varying degrees of \gls{SIMD} parallelism} \om{(which is often smaller than the DRAM row granularity)}, \gfi{\gls{PuD}}  execution \om{often} leads
to \underutilization, throughput loss, and energy waste. 
Second, due to \om{the} \gfcri{high area cost of implementing} \om{interconnects} that connect \gfcri{columns in a wide DRAM row}\revdel{ \gf{in} a DRAM \gfcri{subarray}}, 
most \gfi{\gls{PuD}}  architectures are limited to the execution of \gfcr{parallel} map operations\gfcri{,} where \gfcrii{a single \omii{operation} is performed over equally-sized input and output arrays}.
\gf{Third, the \gfcri{need to feed the wide DRAM row with \omii{tens of} thousands of data \gfcrii{elements} \gfcri{combined with the} lack \gfi{of \om{adequate} compiler support for \gfi{\gls{PuD}}} \gfcrii{systems create a {programmability barrier}}, since \om{programmers} need to {manually} extract \gls{SIMD} parallelism from an application and map computation to the  \om{\gls{PuD}} \gfi{hardware}.}}

Our \textbf{goal} is to design a flexible \gls{PuD} system that overcomes the\revdel{ three} limitations caused by the large and rigid granularity of \gls{PuD}. To \om{this end}, we propose \prop, a hardware/software co-designed \gls{PuD} system that introduces new mechanisms to allocate and control {only} the \om{necessary}\revdel{ computing} resources for \om{a given} \gls{PuD} \omiii{operation}. 
The key idea of \prop is to leverage fine-grained DRAM (i.e., the ability to \omii{independently} access \omi{smaller} \gfcri{segments} of a \omi{large} DRAM row) for \gls{PuD} \omi{computation}. \changeD{\#D1}\revD{\prop \gfcrii{exploits this key idea to} enable a \gfcri{\gls{MIMD}} execution model \om{in each} DRAM \om{subarray} (and \gls{SIMD} execution within each \gfcri{DRAM \omi{row}} segment).} 
\revdel{On the hardware side, \prop does simple changes to 
\li~DRAM's row access circuitry to enable concurrent execution of \gls{PuD} operations in segments of the DRAM row; and 
\lii~to the\revdel{ local and global} DRAM I/O circuitry to allow data to move across DRAM columns \revD{(enabling native support for \gls{PuD} reduction operations)}. 
On the software side, \prop implements compiler passes to 
\li~identify and generate \gls{PuD} operations with the appropriate \gls{SIMD} granularity; and 
\lii~schedule the concurrent execution of independent \gls{PuD} operations.}
%
% We evaluate \prop's performance and energy efficiency using a wide range of real-world applications. Our evaluations show that \prop provides \add{}$\times$ and \add{}$\times$ the performance, and \add{}$\times$ and \add{}$\times$ the energy efficiency of a CPU and a state-of-the-art \gfi{\gls{PuD}}  framework (SIMDRAM), respectively, over \add{} applications while incurring an \add{}\% area overhead on top of a DRAM chip.

We evaluate \prop using \gfcrii{twelve} real-world applications \gfcrii{and 495 multi-programmed application mixes}. 
Our evaluation shows that \prop  \gfcri{\om{provides} 34$\times$ the performance, \efficiencysimdram the energy efficiency, 1.7$\times$ the throughput, and 1.3$\times$ the fairness of a state-of-the-art \gfi{\gls{PuD}}  framework\omi{, along with}} 
\efficiencycpu \gfcri{and} \efficiencygpu the energy efficiency of a high-end CPU \gfcri{and} GPU, \gfcri{respectively}. \prop \gfi{adds} \om{small} area cost \om{to} a DRAM chip (1.11\%) and CPU die (0.6\%). \omi{We hope and believe that \prop's ideas and results will help \omii{to enable} more efficient and easy-to-program \gls{PuD} systems. \omii{To this end, we open source} \prop at \url{https://github.com/CMU-SAFARI/MIMDRAM}.}
 
 % \add{}$\times$ and \add{}$\times$ the performance, and \add{}$\times$ and \add{}$\times$ the energy efficiency of a CPU and a state-of-the-art \gfi{\gls{PuD}}  framework (SIMDRAM), respectively, over \add{} applications while incurring an \add{}\% area overhead on top of a DRAM chip.

% Processing-using-DRAM is an emerging \gls{PIM} approach that leverages DRAM's massive internal parallelism to execute bulk data copy, bitwise, and arithmetic operations. % (i.e., at the granularity of a DRAM row, usually \SI{8}{\kilo\byte} or 65'536 data-parallel operands). 
% However, the \emph{large} and \emph{rigid} granularity \juan{of} 
% %that 
% DRAM rows
% %are activated to execute \gfi{\gls{PuD}}  computation 
% limit the effectiveness and applicability of \gfi{\gls{PuD}}  architectures in \gf{two} ways. 
% First, since real applications display \emph{varying} degrees of \juan{SIMD parallelism}, 
% %bulk parallelism, 
% \gfi{\gls{PuD}}  execution \juan{frequently leads} %can lead 
% to under-utilization, throughput loss, and energy waste. % when there is a mismatch between the degree of data parallelism an application presents and the execution granularity of the \gfi{\gls{PuD}}  substrate.
% %\gf{Second, programming the ultra-large \gfi{\gls{PuD}}  SIMD substrate becomes a hard task since, due to a lack of automated tools and compilers for \gfi{\gls{PuD}}  architectures, the programmer needs to \emph{manually} \li~identify, map, and orchestrate the available SIMD parallelism in general-purpose applications and map . }
% Second, due to the \juan{lack of} 
% %cost of implementing 
% interconnect networks that connect DRAM columns inside a DRAM array,
% %to support data movement across %a large number of DRAM columns inside a DRAM array, 
% most \gfi{\gls{PuD}}  architectures are limited to the execution of embarrassingly parallel map operations.% (i.e., there is \emph{no} native support for reduction operations).   

%and 
%\lii~the need to \emph{manually extract} a massive amount of data parallelism from an application to satisfy the large granularity execution model of the \gfi{\gls{PuD}}  architecture. %maximize  lack of programming models and compilers for the execution of general-purpose applications in the \gfi{\gls{PuD}}  architecture. 

% for two reasons. 
% First, the \gfi{\gls{PuD}}  architecture's bulk parallelism is often only partially utilized when an application is not embarrassingly parallel (i.e., when the total number of operands used during the execution of an \gfi{\gls{PuD}}  operation is lower than the DRAM row size), causing sub-optimal performance and wasted energy consumption. Second, due to a lack of programming models and compilers for general-purpose \gfi{\gls{PuD}}  architectures, the programmer needs to manually extract a large amount of data-level parallelism from the application to be mapped to the underlying DRAM substrate, which can be challenging. 

%Our \emph{goal} in this work is to enhance state-of-the-art \gfi{\gls{PuD}}  substrates with solutions to increase utilization and automate programmability.

%Our \emph{goal} is to design a flexible yet simple \gfi{\gls{PuD}}  substrate that overcomes the two limitations caused by the large and rigid granularity of \gfi{\gls{PuD}}  execution. To do so, we propose \prop, a hardware/software co-designed \gfi{\gls{PuD}}  substrate that introduces the ability to allocate and control \emph{only} the needed computing resources for \gfi{\gls{PuD}}  computation. The key idea of \prop is to leverage fine-grained DRAM access/activation (i.e., the ability to access/activate only portions of a DRAM row) for \gfi{\gls{PuD}}  operations. %Prior works on fined-grained DRAM accesses/activation propose simple modifications to the DRAM access circuitry to enable loading only portions of the DRAM row, which can improve overall energy efficiency. In \prop, we exploit such solutions to allow the individual execution of \gfi{\gls{PuD}}  operations in the appropriate portion of the DRAM row, which enables a \gls{SIMD} and \gls{MIMD} execution models within the DRAM array. 

% Our \emph{goal} in this work is to design a flexible yet simple \gfi{\gls{PuD}}  substrate that overcomes the two limitations caused by the large and rigid granularity of \gfi{\gls{PuD}}  execution. To do so, we propose \prop, a hardware/software co-designed \gfi{\gls{PuD}}  substrate that introduces \juan{new mechanisms} %the ability 
% to allocate and control \emph{only} the needed computing resources for \gfi{\gls{PuD}}  computation. The key idea of \prop is to leverage fine-grained DRAM access (i.e., the ability to access only portions of a DRAM row) for \gfi{\gls{PuD}}  operations. %\prop leverage such a key idea in both hardware and software. 
% On the hardware side, \prop proposes simple modifications to
% \li~the DRAM access circuitry of %a few 
% DRAM rows to enable the \juan{independent} 
% %individual 
% and \juan{concurrent} execution of \gfi{\gls{PuD}}  operations in segments of the DRAM row; and 
% \lii~to the local and global DRAM I/O circuitry to allow data to move across DRAM columns at different granularities. With such modifications, \prop enables a \gls{MIMD} execution model in a single DRAM array \juan{and natively supports} %while natively supporting 
% the execution of \gfi{\gls{PuD}}  reduction operations. 
% %
% % includes 
% % \li~a latch in a small subset of the DRAM array's accessing circuitry to enable the individual execution of \gfi{\gls{PuD}}  operations in segments of the DRAM row; and 
% % \lii~a low-cost control unit placed in the memory controller that transparently orchestrates the concurrent execution of independent \gfi{\gls{PuD}}  operations within a single DRAM row. 
% On the software side, \prop \gf{implements} compiler passes to 
% \li~identify and generate the \gfi{\gls{PuD}}  operations for \gfi{\gls{PuD}} -friendly code regions with the appropriate computation granularity; and
% \liii~schedule the concurrent execution of independent \gfi{\gls{PuD}}  operations to maximize \gf{overall} utilization.% of the \gfi{\gls{PuD}}  substrate.

% We evaluate \prop's performance and energy efficiency using a wide range of real-world applications. Our evaluations show that \prop provides \add$\times$ and \add$\times$ the performance, and \add$\times$ and \add$\times$ the energy efficiency of a CPU and a \juan{state-of-the-art \gfi{\gls{PuD}}  framework (SIMDRAM), respectively}, over \add{} applications, while incurring on \add\% area overhead on top a DRAM chip. 

\end{abstract}


==> mainmatter/05_mimdram/sections/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\glsresetall

\omi{\emph{Data movement} between computation units (e.g., CPUs, GPUs) and  main memory (e.g., DRAM) is a major \emph{performance} and \emph{energy bottleneck} in current computing systems~\gfcri{\cite{
mutlu2013memory,
mutlu2015research,
dean2013tail,
kanev_isca2015,
mutlu2019enabling,
mutlu2019processing,
mutlu2020intelligent,
ghose.ibmjrd19,
mutlu2020modern,
boroumand2018google, 
wang2016reducing, 
mckee2004reflections,
wilkes2001memory,
kim2012case,
wulf1995hitting,
ghose.sigmetrics20,
ahn2015scalable,
PEI,
sites1996,
deoliveira2021IEEE}}, and is expected to worsen due to the increasing data intensiveness of modern applications~\cite{sevilla2022compute,gholami2020ai_and_memory_wall}.} 
To mitigate the overheads \sg{caused by data movement}, several works propose \gls{PIM} architectures~\gfcriii{\pim}\revdel{, where computation is moved \juan{closer to}~\pnm or \omi{inside}~\pum memory \om{chips}}.
\gfcri{There are two main approaches to \gls{PIM}~\cite{ghose.ibmjrd19, mutlu2020modern}:
\li~\gls{PnM}~\gfcriii{\pnm}, where \omi{computation} logic is added \omi{near} the \omi{memory arrays (e.g., in a DRAM chip or at the logic layer of a 3D-stacked memory~\cite{HMC2, HBM,lee2016simultaneous})}; and
\lii~\gls{PuM}~\pum, where computation is performed by exploiting the analog operational properties of the memory \omi{circuitry}.}
%
\gfcrii{There are two main advantage\gfcrii{s} of \gls{PuM} \omi{over} \gls{PnM}. First, \gls{PuM}  \emph{fundamentally} \emph{eliminates} data movement by performing computation \emph{in situ}, while data movement still occurs between computation units and memory arrays in \gls{PnM}.} 
Second, \gls{PuM} architectures \omi{exploit}  the large internal bandwidth and parallelism available \omi{\emph{inside}} the memory arrays, while \gls{PnM} solutions are \emph{fundamentally} bottlenecked by the memory's internal data buses.

\gfcri{\gls{PuM} architectures can be implemented using different memory technologies\omi{,} including} SRAM~\gfcriii{\srampum}, DRAM~\drampum, emerging non-volatile~\gfcriii{\nvmpum} or \omi{NAND} flash~\gfcriii{\flashpum}.
\gfi{\gls{PuD}}~\drampum, \gfi{in \sg{particular}}, \gfcri{enables the execution of different \emph{bulk} operations in DRAM (i.e., \gls{PuD} operations), such as 
\li~data copy \gfcri{and initialization}~\cite{seshadri.bookchapter17, seshadri2013rowclone,seshadri2018rowclone,chang2016low},
\lii~\om{bitwise} Boolean operations~\cite{seshadri2017ambit, gao2019computedram, xin2020elp2im, besta2021sisa, li2017drisa}, 
\liii~arithmetic operations~\cite{deng2018dracc, gao2019computedram,li2017drisa,angizi2019graphide, hajinazarsimdram,li2018scope}, and 
\liv~lookup table \omi{based} operations~\gfcri{\cite{ferreira2021pluto,ferreira2022pluto,deng2019lacc,sutradhar2021look,sutradhar2020ppim}}}. 

%Based on these prior works, follow-up proposals have implemented frameworks that extend the functionalities of \gls{PuM} architectures by constructing new and more complex operations. For example, SIMDRAM~\cite{hajinazarsimdram}, which leverages a \gfi{\gls{PuD}} substrate proposed by Ambit~\ambit, designs a three-step methodology that allows the user to implement \emph{any} complex \gfi{\gls{PuD}} operation by orchestrating sequences of DRAM commands. 
\gfcrii{\gfi{\gls{PuD}} architectures commonly employ bit-serial computation~\cite{angizi2019graphide,besta2021sisa,gao2019computedram,seshadri.bookchapter17, seshadri2013rowclone,seshadri2015fast,seshadri2016buddy, seshadri2016processing, seshadri2017ambit,seshadri2018rowclone, seshadri2019dram, xin2020elp2im, hajinazarsimdram}, where they map \gfcrii{each data element} of a \gls{PuD} operation to a DRAM column.\footnote{\gfcri{We provide a detailed background on DRAM organization in \cref{sec:background:dram}.}} 
\gfcrii{\omi{A} \gls{PuD} architecture that leverages bit-serial computation effectively enables a very-wide \gls{SIMD} execution \gfcrii{model} in DRAM, with a \emph{large} and \emph{rigid} computation granularity.}
\gfcrii{The \emph{large} computation granularity stems from the fact that} bit-serial computation turns each one of the \emph{many}
DRAM columns in a DRAM subarray into a computing engine.
For example, there are \gfcrii{16,384--262,144} DRAM columns in a \gfcrii{DDR4 DRAM~\cite{micron2014ddr4} subarray}, and each can execute \gfcrii{a \emph{single} \gls{PuD} operation over \emph{multiple} data elements stored on the DRAM columns.} 
\gfcrii{The \emph{rigid} computation granularity stems from the fact that} the granularity \omii{at} which DRAM rows are accessed dictates the computation granularity of a \gls{PuD} operation. 
In commodity DRAM chips, all DRAM row accesses happen at a \emph{fixed} granularity\omi{:} the DRAM access circuitry addresses \emph{\omi{all}} DRAM columns in a DRAM row \emph{simultaneously}. As such, \emph{every} \gls{PuD} operation operates simultaneously on \emph{all} the 16,384 to 262,144 data elements (one per DRAM column) a DDR4 DRAM subarray stores, for example.}

%\gfi{\gls{PuD}} operations are executed in a \gls{SIMD} manner by storing all bits of a operand vertically in a single column of a DRAM array. 
\revdel{In this execution model, the \gfhpca{granularity where DRAM rows are opened (i.e., activated)} fixed size of the DRAM row (e.g.,  \SI{8}{\kilo\byte} in DDR4 DRAM~\cite{standard2012jesd79}) defines the \gfi{computation granularity}.}
% of the \gls{SIMD} computation \gf{(i.e., the \gls{SIMD} width)}. 
%Similar \gls{PuM} frameworks have been proposed for other memory substrates, such as Duality Cache~\cite{dualitycache}, which enables a \gls{SIMT} execution model in a  processing-using-cache substrate, and IMP~\cite{fujiki2018memory}, which enables a \gls{SIMD} execution model in a processing-using-NVM substrate.

% \gfi{Many of these} \gls{PIM} architectures \gf{implement computation by manipulating the operation of SRAM~\srampum, DRAM~\drampum, emerging non-volatile~\nvmpum or flash~\flashpum memory cells. These \gls{PIM} architectures \juani{are referred to as} \gls{PuM}~\pimdef.}
% can be broadly divided into two main categories~\pimdef: 
% \li~\gls{PuM}~\pum, where computation is performed by manipulating the operation of memory cells, and
% \lii~\gls{PnM}~\pnm, where computation is performed by adding logic elements into the same package/chip/bank/array as memory. The primary benefit of \gls{PuM} in comparison with \gls{PnM} is that the former can \emph{fully} leverage the abundant memory bandwidth and parallelism available inside the memory. In contrast, the latter is \emph{fundamentally} bounded by the memory's internal interconnections.
%
% Many works~\cite{angizi2019graphide,besta2021sisa,bostanci2022dr,deng2018dracc,ferreira2021pluto,ferreira2022pluto,gao2019computedram,li2017drisa,li2018scope,olgun2021quactrng,olgun2022pidram,seshadri.bookchapter17, seshadri2013rowclone,seshadri2015fast,seshadri2016buddy, seshadri2016processing, seshadri2017ambit,seshadri2018rowclone, seshadri2019dram, xin2020elp2im,aga2017compute,eckert2018neural,si2019dual,simon2020blade,nag2019gencache,wang2019bit,flashcosmos,gao2021parabit} have demonstrated how 
%Different memory technologies can be manipulated to implement \gls{PuM}, including  SRAM~\srampum, emerging non-volatile memories~\nvmpum, and flash~\flashpum. 
%



\sg{We highlight three limitations} of state-of-the-art \gfi{\gls{PuD}} architectures that stem from the \emph{large} and \emph{rigid} granularity of \gfhpca{\gls{PuD}'s \om{very}-wide \gls{SIMD} execution model.} 
%\juan{DRAM rows}. 
First, to \revdel{make \juan{efficient} use of the %bulk \gls{SIMD} 
parallelism available inside DRAM and }sustain high \omii{\emph{\gls{SIMD} utilization}} \gfcri{(i.e., the fraction of \gls{SIMD} lanes executing a useful operation)}, \om{each} \gfi{\gls{PuD}} \om{operation needs to operate on} a \emph{large} amount of data. \om{Unfortunately, not all applications \omii{have} the required large amount of data parallelism to sustain high \gls{SIMD} utilization in \gls{PuD} architectures. Our} analysis of \gfcrii{twelve} general-purpose  applications \gfcrii{(compiled for a high-end CPU system)} shows that the degree of \gls{SIMD} parallelism an application \gfcrii{has} \emph{varies} significantly, from as low as 8 to as high as 134,217,729 \omi{data elements} per \gls{SIMD} instruction (\cref{sec:motivation}). 
Second, the large granularity of \gfi{\gls{PuD}} execution makes \sg{it \gfcri{costly} to implement} \gfcri{interconnects that connect columns in a DRAM row. \gfcri{Such \omi{interconnects} could allow for the implementation of}} \gfi{\gls{PuD}} operations that require \gfcri{shifting data across DRAM columns, which is a common computing pattern present in vector-to-scalar reduction operations, \omi{e.g.,} \texttt{sum += A[i]}}. This \sg{limits} \gfi{\gls{PuD}} operations to \emph{only} parallel map operations \gfcri{(i.e., operations where an output data of the same \omi{dimension} as the input data is produced by applying a computation \omi{independently} to each input operand)}. \gfcri{\gfi{A} prior work~\cite{li2017drisa} proposes modifications to the DRAM array to enable communication across DRAM columns\gfi{. However,} \juani{the \omi{interconnection network that this work proposes can lead} to prohibitive area \gfi{cost} \omi{in} commodity DRAM \omi{chips} \gfcri{(i.e., 21\% DRAM area overhead, see \cref{sec:eval:otherpims})}.}} 
\gfcri{Third, the need to feed a \omii{very-}wide DRAM
row with thousands of data \gfcrii{elements} combined with the
lack of adequate compilation tools that can identify very-wide \gls{SIMD}  instructions in general-purpose applications and map such instructions to equivalent \gls{PuD} operations create a \emph{programmability barrier} for \gls{PuD} architectures. In state-of-the-art \gls{PuD} architectures~\gfcrii{\cite{angizi2019graphide,besta2021sisa,bostanci2022dr,deng2018dracc,ferreira2022pluto,gao2019computedram,li2017drisa,li2018scope,olgun2021quactrng,olgun2022pidram, seshadri2013rowclone, seshadri2016processing, seshadri2017ambit, seshadri2019dram, xin2020elp2im, hajinazarsimdram}}, the programmer needs to \emph{manually} extract a \emph{large} and \emph{fixed} amount of data-parallelism from an application and map computation to the underlying \gls{PuD} hardware, which is a daunting task.}
% GF: The problem definition needs to be improved. Follow the abstract. Make the first issue related to the rigid granularity of a \gfi{\gls{PuD}} operation (i.e., always at the granularity of a DRAM row). This is an issue for at least two main reasons. First, applications have varying amount of SIMD parallelism, ranging from subsets of a DRAM row to multiples of a DRAM row. When subsets of a DRAM row are required, the overall architecture suffers from under-utilization. Second, the rigid granularity limits the type of computation patterns that can be executed within DRAM. Limited to map operations since there is no interconnection path across DRAM rows, and implementing such interconnection can lead to prohibitive area overheads. This is a particular problem for applications that rely on reduction operations, since reductions need to be executed by the host CPU. 
%First, to make effective use of the bulk \gls{SIMD} parallelism available inside DRAM and sustain high \gls{SIMD} utilization of the \gfi{\gls{PuD}} substrate, the programmer needs to \emph{manually} extract a large amount of data parallelism (i.e., at least 65'536 data-independent operands, where each operand is mapped to a column of a DRAW row) from the application. However, our analysis of a wide range of general-purpose applications (Section~\ref{sec:motivation}) shows that the amount of data parallelism within an application varies significantly. This means that the maximum \gls{SIMD} width (i.e., the number of independent working items in an \gfi{\gls{PuD}} operation) that can be exploited for a particular \gfi{\gls{PuD}} operation also varies, from larger multiples of the DRAM row size (leading to high \gls{SIMD} utilization of the \gfi{\gls{PuD}} substrate) to subsets of a DRAM row (leading to low \gls{SIMD} utilization). The resulting SIMD under-utilization can lead to energy and throughput waste since costly DRAM operations are performed over portions of the DRAM row that does \emph{not} contain useful data (e.g., they are padded with zeros). 

%The \emph{second limitation} is caused by a \emph{lack of programming support} for \gfi{\gls{PuD}} substrates, which makes extracting data parallelism and modifying an application to use \gfi{\gls{PuD}} operations daunting. 
%To map a particular application to the \gfi{\gls{PuD}} substrate, the programmer needs to manually
%\li~identify appropriate regions of the application that could benefit from \gfi{\gls{PuD}} execution;
%\lii~extract as much data parallelism as possible (using techniques such as loop unrolling), aiming to exploit the \emph{SIMD} parallelism of \gfi{\gls{PuD}} subtract entirely; and
%\liii~mark the data structures involved in the \gfi{\gls{PuD}} computation to guarantee data consistency and coherence.

%Second, due to a \emph{lack of programming support} for \gfi{\gls{PuD}} substrates, extracting data parallelism and modifying an application to use \gfi{\gls{PuD}} operations is daunting. To map a particular application to the \gfi{\gls{PuD}} substrate, the programmer needs to manually
%\li~identify appropriate regions of the application that could benefit from \gfi{\gls{PuD}} execution;
%\lii~extract as much data parallelism as possible (using techniques such as loop unrolling), aiming to exploit the SIMD parallelism of \gfi{\gls{PuD}} subtract entirely; and
%\liii~mark the data structures involved in the \gfi{\gls{PuD}} computation to guarantee data consistency and coherence.

Our \emph{goal} is to design a flexible \gfi{\gls{PuD}} substrate that overcomes the \gf{three} limitations caused by the large and rigid granularity of \gfi{\gls{PuD}} execution. To \om{this end}, we propose \prop, a hardware/software co-designed \gfi{\gls{PuD}} \gfi{system} that introduces the ability to allocate and control \emph{only} the \om{required amount of} computing resources inside the DRAM \gfcri{subarray} for \gfi{\gls{PuD}} computation. The \emph{key idea} of \prop is to leverage fine-grained DRAM for \gfi{\gls{PuD}} operations. 
Prior works on fine-grained DRAM~\gfcriii{\cite{cooper2010fine,udipi2010rethinking,zhang2014half,ha2016improving,lee2017partial,olgun2022sectored,o2021energy,oconnor2017fine}} \gfcri{leverage the hierarchical design of a DRAM subarray \gfcrii{to enable DRAM row accesses with \emph{flexible} granularity. A DRAM subarray is composed of multiple (e.g., \gfcrii{32--128}) smaller 2D arrays of \gfcrii{512--1024} DRAM rows and \gfcrii{512--1024} columns, called \emph{DRAM mats}~\cite{standard2012jesd79,seshadri2019dram,seshadri2016processing,zhang2014half}.
\gfcrii{During a row access, the DRAM access circuitry \emph{simultaneously} addresses \emph{all} columns across \emph{all} mats in a subarray, composing a \emph{large} DRAM row of size \texttt{[\#columns\_per\_mat $\times$ \#mats\_per\_subarray]}.
Fine-grained DRAM \omiii{modifies} the DRAM access circuitry to}} enable reading/writing data \omi{from/}to \gfcri{individual DRAM mats}, allowing the access of DRAM rows with a \omii{smaller} number of columns. } 

\gfcrii{Inspired by fine-grained DRAM, we propose
simple modifications to the DRAM access circuitry to enable
addressing individual DRAM mats during \gls{PuD} computation.
Fine-grained DRAM for \gls{PuD}  computation brings four main advantages. 
First, by addressing individual DRAM mats, \prop better matches the granularity of a \gls{PuD} operation to the available data-parallelism \omii{present in} the application.
Second, with fewer DRAM columns per \gls{PuD} operation, \prop makes it feasible to implement low-cost interconnects inside a DRAM subarray, allowing for data movement \emph{within} and \emph{across} DRAM mats.
Third, since the number of columns in a single DRAM mat
is on par with the number of \gls{SIMD} lanes in modern processors' \gls{SIMD} engines  (e.g., 512 \gls{SIMD} lanes in  AVX-51 \gls{SIMD} engines2~\cite{firasta2008intel}), \prop can leverage
traditional compilers to map \gls{SIMD} instructions to \gls{PuD} operations.
Fourth, \prop leverages \emph{unused} DRAM
mats to \omii{\emph{concurrently}} execute \emph{independent} \gls{PuD} operations
\emph{across} DRAM mats in a \emph{single} DRAM subarray. This enables the \gls{PuD} substrate to execute a \emph{not-so-wide} \gls{PuD} \omii{operation} in a subset of the DRAM mats and other independent \gls{PuD} operations across the remaining DRAM mats within a single DRAM subarray, in a \gls{MIMD} fashion~\cite{smith1986pipelined,flynn1966very,thornton1964parallel}.}



% \revD{This opens up a new opportunity for \gls{PuD} \omi{computation}: by leveraging the unused \gfcri{segments} of \gfcri{a} DRAM row \gfcri{across different DRAM mats}, the \gls{PuD} substrate can execute \emph{multiple} \gls{PuD} \gfcri{operations} over \emph{multiple} input data \emph{concurrently} in a single DRAM \gfcri{subarray}. \gfcri{Practically allowing \prop to execute \gls{PuD} operations} in a \gls{MIMD} fashion~\cite{smith1986pipelined,flynn1966very,thornton1964parallel}.
%can execute data-independent \gls{SIMD}operations within the DRAM array in a \gls{MIMD} fashion. This way, different portions of a DRAM array can execute \emph{multiple} \gls{PuD} \gls{SIMD} \gfhpca{instructions} over \emph{multiple} input data concurrently, improving throughput and utilization.


%, enabling a \gls{MIMD} execution model within the DRAM array, where different portions of a DRAM array execute multiple \gfi{\gls{PuD} \gls{SIMD}} operations over multiple input data concurrently. 

\prop leverages fine-grained DRAM for \gfi{\gls{PuD}} in hardware and software. On the hardware side, \prop \gf{proposes simple modifications to the DRAM \gfcri{subarray} and includes new mechanisms to the memory controller that allow the execution of \gfcri{independent} \gfi{\gls{PuD}} \gfcri{operations across the DRAM mats in a single  subarray}.  Concretely, \gfcrii{\prop includes}}  
\li~latches, isolation transistors, and selection logic in the DRAM \gfcri{subarray}'s \gfcri{access} circuitry to enable the execution of \gfcrii{independent} \gfi{\gls{PuD}} \gfcri{operations \omi{in} different DRAM mats}; 
\lii~two different low-cost \gfcri{interconnects} placed \omi{respectively} at the local and global DRAM I/O circuitry\sg{, which enable communication} across columns of a DRAM row at varying granularities \gfcr{and} \revdel{\sg{allowing for} }the execution of vector\gfcri{-to-scalar} reduction \gfcri{in DRAM} at low \omi{hardware} cost. 
\gf{\omii{In} the memory \sg{controller}, \prop includes a new control unit that orchestrates the concurrent execution of \gfcri{independent} \gfi{\gls{PuD}} \gfcri{operations} \gfcri{\omii{in} different \omii{mats} of a DRAM subarray}.} 
On the software side, \prop \gfi{implements} compiler passes to
\li~automatically vectorize code regions that can benefit from \gfi{\gls{PuD}} execution \omi{(called \gls{PuD}-friendly regions)};
\lii~\omi{for such regions,} generate \gfi{\gls{PuD}} \gfcri{operations} with the most appropriate \gls{SIMD} granularity; and
\liii~schedule the concurrent execution of \gfcri{independent} \gfi{\gls{PuD}} \gfcri{operations \omi{in} different DRAM mats}. \gf{\gfcri{W}e discuss how to integrate \prop in a real system\gfcr{, including how \prop deals with 
\li~data allocation \gfcri{\omi{within} a DRAM subarray} and 
\lii~mapping \gfcri{of \omi{a} \gls{PuD}'s operands to guarantee high utilization of the \gls{PuD} substrate\revdel{ and low data movement across DRAM mats}.}}}

We evaluate \prop's \gf{\gfcri{performance, energy efficiency, throughput, fairness}\gf{, and \gf{SIMD utilization}}} for \gfcri{twelve} real-world applications from four popular benchmark suites (i.e., Phoenix~\cite{yoo_iiswc2009}, Polybench~\cite{pouchet2012polybench}, Rodinia~\cite{che_iiswc2009}, and SPEC 2017~\cite{spec2017}) \gfcri{and 495 multi-programmed application mixes}. 
Our evaluation shows that \prop \om{provides} \gfcri{34$\times$ the performance}, \efficiencysimdram the energy efficiency, 1.7$\times$ the throughput, 1.3$\times$ the fairness, \gfcri{and 18.6$\times$ the \gls{SIMD} utilization} of \gfcri{SIMDRAM~\cite{hajinazarsimdram}} (a state-of-the-art \gfi{\gls{PuD}} framework); \gfcri{while providing} \efficiencycpu and \efficiencygpu the energy efficiency of a high-end CPU \gfcri{and GPU, respectively}. 
\gfcri{\omii{MIMDRAM}\omi{'s improvements are}  due to its ability to 
\li~maximize the utilization of the  \gls{PuD} substrate by \emph{concurrently} \omi{executing} independent \gls{PuD} operations within \omi{each} DRAM subarray, and 
\lii~allocate \emph{only} the necessary resources (i.e., \gfcrii{appropriate number of DRAM mats}) for a \gls{PuD} operation.}
\prop \gfcri{adds small} area cost \gfcri{to} a \gfcri{state-of-the-art} DRAM chip (1.11\%) and \gfcri{state-of-the-art} CPU die (0.6\%).

We make the following key contributions:
\begin{itemize}[leftmargin=3mm,itemsep=0mm,parsep=0mm,topsep=0mm]
\item To our knowledge, this is the first work to propose \juani{an end-to-end} \gfcri{processing-using-DRAM (PUD)} \omi{system} for general-purpose applications\omi{,} \gfcri{\omi{which} executes operations in a multiple-instruction multiple-data (MIMD) fashion}. \prop \omi{makes} low-cost modifications to the DRAM \gfcri{subarray design that enable the} \gfcri{\emph{concurrent}} \gfcri{execution of} \gfcri{multiple} \gfcri{independent} \gfi{\gls{PuD}} \gfcri{operations} in a single DRAM \gfcri{subarray}. 

\item We propose compiler passes that \gfcri{\omii{take} as input unmodified C/C++ applications and,} transparently \omii{to} the \gfcri{programmer}, 
\li~identify \gfcri{loops \omi{that are}} \gfcri{suitable} for \gfi{\gls{PuD}} execution,
\lii~transform the \gfcri{source} code to use \gfi{\gls{PuD}} \gfcri{operations}, and \liii~schedule \gfcri{independent \gls{PuD} operations for concurrent execution \omi{in each DRAM subarray}, maximizing \gfcri{utilization} \omi{of} the underlying \gls{PuD} architecture}. 

\item We evaluate \prop with a wide range of general-purpose applications and observe that \omi{it} provides higher energy efficiency \omi{and} system throughput than state-of-the-art \gfi{\gls{PuD}}\gfcri{, CPU, and GPU architectures}. 

\item \gfcrii{We open-source \prop  at \url{https://github.com/CMU-SAFARI/MIMDRAM}}.
\end{itemize}

==> mainmatter/05_mimdram/sections/02_background.tex <==
\section{Background}
\label{sec:background}

We first briefly explain the architecture of a typical DRAM chip.\footnote{We refer the reader to \omii{various} prior works~\gfcriii{\drambackgroundshort}~for a more detailed description of the DRAM architecture.} Second, we describe prior \gls{PuD} works that \prop builds on top of. 

% \gf{We briefly explain 
% \li~the architecture of a typical DRAM chip, and 
% \lii~prior processing-using-DRAM \gfi{(PuD)} works.}

% {\color{red} \rule{\linewidth}{0.5mm} \\ \textbf{V3 STALE TEXT BEGIN} \\ \rule{\linewidth}{0.5mm}}

\subsection{DRAM Organization \& \juan{Operation}}
\label{sec:background:dram}

\paratitle{DRAM Organization} A DRAM system comprises \omi{of} a hierarchy of components, as \gfi{Fig.}~\ref{fig_subarray_dram} illustrates\revdel{, starting with a DRAM module at the highest level}. 
A \emph{DRAM module} (\gfi{Fig.}~\ref{fig_subarray_dram}a) \gfi{has} several (e.g., 8--16) DRAM chips. 
A \emph{DRAM chip} (\gfi{Fig.}~\ref{fig_subarray_dram}b) \gfi{has} multiple DRAM banks (e.g., 8--16). 
A \emph{DRAM bank} (\gfi{Fig.}~\ref{fig_subarray_dram}c) \gfi{has} multiple (e.g., 64--128) 2D arrays of DRAM cells known as \emph{DRAM mats}. Several DRAM mats (e.g., 8--16) are grouped in a \emph{DRAM subarray}. \gfcrii{In a DRAM bank, there are three global components that are used
to access the DRAM mats (as Fig.~\ref{fig_subarray_dram}c depicts):}
%three global components are used to access columns of the mats \gfi{in} a subarray:
\li~a \emph{global row decoder} that selects a row of DRAM cells \emph{across} multiple mats \omi{in a subarray},
\lii~a \emph{column select logic} (CSL) that selects portions of the DRAM row based on the column address, and
\liii~a \emph{global sense amplifier} \omi{(i.e., global row buffer)} that transfers the selected fraction of the data from the \omi{selected} DRAM row through the \emph{global \omi{bitlines}}.

A \emph{DRAM mat} (\gfi{Fig.}~\ref{fig_subarray_dram}d) \omi{consists of a 2D array of} DRAM cells \omi{organized} into multiple \emph{rows} (e.g., 512--1024) and multiple \emph{columns} (e.g., 512--1024)~\cite{kim2018solar, lee2017design, kim2002adaptive}. 
A \emph{DRAM cell} (\gfi{Fig.}~\ref{fig_subarray_dram}e) consists of an \emph{access transistor} and a \emph{storage capacitor}. 
%that encodes a single bit of data using its voltage level. 
The source nodes of the access transistors of all the DRAM cells in the same column connect the cells' storage capacitors to the same \emph{local bitline}. The gate nodes of the access transistors of all the DRAM cells in the same row connect the cells' access transistors to the same \emph{local wordline}. Each mat contains 
\li~a \emph{local row decoder} that drives the local wordlines to the appropriate voltage levels to \gfcr{open (activate)} a row, 
\lii~a row of sense amplifiers (also called a \emph{local row buffer}) that senses and latches data from the activated row, and
\liii~\emph{\glspl{HFF}} that drive a portion (e.g., \SI{4}{\bit}) of the data \gfi{in} the local row buffer to the global \omi{bitlines}. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/dram_subarray-crop.pdf}
    \caption{\gfcrii{\omii{Overview} of DRAM organization.}}
    \label{fig_subarray_dram}
\end{figure}

\paratitle{DRAM \juan{Operation}} Three major steps are involved in serving a main memory request. First, to select a DRAM row, the memory controller issues an \texttt{ACTIVATION} (\texttt{ACT}) command with the row address. On receiving this command, \omi{the} DRAM \omi{chip transfers} all the data in the row to the corresponding local row buffer. \revdel{The two-terminal sense amplifier in the local row buffer connected to each local bitline senses the voltage difference between the local bitline and a reference voltage and amplifies it to a CMOS-readable value.} %In doing so, the sense amplifier connected to the reference voltage is amplified to the \emph{opposite} (i.e., \emph{negated}) value. 
%The local row buffer maintains the sensed data for as long as the row is \emph{open} (i.e., the local and global wordlines continue to be asserted).
Second, to access a cache line from the activated row, the memory controller issues a \texttt{READ} (\texttt{RD}) command with the column address of the request. \revdel{ DRAM then transfers portions of the selected data from the local row buffer in each mat to the global row buffer (via the \glspl{HFF}) of the DRAM bank and from the DRAM bank to the memory controller over the memory channel.} Third, to enable the access of another DRAM row in the same bank, the memory controller issues a  \texttt{PRECHARGE} (\texttt{PRE}) command with the address of the currently activated \gfi{DRAM bank}. This command disconnects the local bitline by disabling the local wordline, and the local bitline voltage is restored to its quiescent state.% (e.g., typically $\frac{1}{2}V_{DD}$). 

%While this is a high-level description of the three major DRAM operations, these operations, in reality, 


%\paratitle{DRAM Timing Parameters} The memory controller manages main memory requests by issuing row and column access commands to DRAM. Internal DRAM operation considerations determine the minimum time between these commands, such as how long it takes to sense data from cells in a selected wordline, and how long it takes to transfer data from the local to the global row buffer~\cite{lee2017design, kim2012case, lee2015adaptive,Tiered-Latency_LEE}. There are three major timing parameters for managing row and column access. \texttt{tRAS} (\texttt{tRP}) is the minimum time needed to select (deselect/precharge) a row in a bank for activation. \texttt{tRCD} is the minimum time required to update the data in a column of a row after activating the row. 

% \paratitle{Coarse-Grained DRAM Access \& Activation} The three major DRAM operations consist of two levels of \emph{coarse-grained activations/accesses} through
% \li~global structures across mats within a bank (global row buffer, global wordlines, and global bitlines) and 
% \lii~local structures within a mat (local row buffer, local wordlines, and local bitlines). A DRAM row-column access goes through multiple steps in the global-local hierarchy, as annotated in \gfi{Fig.}~\ref{fig_subarray_dram}:
% \circled{1} When the global row decoder in a bank receives a row address, it first activates the corresponding global wordline in the bank.
% \circled{2} The global wordline, in turn, activates the corresponding local row decoder in each mat that it is connected to.
% \circled{3} The local row decoder in each mat activates the corresponding local wordline, connecting the row to the local row buffer. A single row address controls a large-size \emph{logical} DRAM row, which spreads across all the mats in a subarray, and across all DRAM chips. A typical \SI{8}{\kilo\byte} size logical DRAM row is composed by addressing simultaneously 512 local bitlines (and thus 512 DRAM cells, each storing a single bit) in a mat across 16 mats in a DRAM subarray and 8 DRAM chips in a DRAM module (\SI{512}{\bit} per mat $\times$ 16 mats per chip $\times$ 8 chips per module = \SI{65536}{\bit} =  \SI{8}{\kilo\byte})~\cite{standard2012jesd79,seshadri2019dram,seshadri.bookchapter17,seshadri2017ambit,seshadri2016processing,zhang2014half}.
% \circled{4} The local row buffer senses and latches the entire row through the local bitlines in each mat across the bank. 
% \circled{5} When the memory controller issues a \texttt{RD} command with the column address of the request, a fraction (e.g., \SI{4}{\bit}) of data from each mat is selected by the column select logic using the column address and transferred from the local row buffer to the global row buffer, through the global bitlines. In a typical DDR4 DRAM  module~\cite{standard2012jesd79,seshadri2019dram,seshadri.bookchapter17,seshadri2017ambit,seshadri2016processing,zhang2014half}, a global row buffer logically latches \SI{64}{\byte} of the activated row, distributed across mats and chips (\SI{4}{\bit} per mat $\times$ 16 mats per chip $\times$ 8 chips per module = \SI{512}{\bit} = \SI{64}{\byte}).
% \circled{6} Data from the global row buffer is then sent to the memory channel through the I/O logic of the DRAM chip. In a typical DRAM, a \texttt{RD} command reads out 8 data beats (also called an 8-beat burst), thus reading a complete \SI{64}{\byte} cache line.


\revdel{\paratitle{Fine-Grained DRAM Access \& Activation} 
%
% \gf{The three major DRAM operations consist of two levels of \emph{coarse-grained activations/accesses} through
% \li~global structures across mats within a bank (global row buffer, global wordlines, and global bitlines) and 
% \lii~local structures within a mat (local row buffer, local wordlines, and local bitlines). %
% During an \texttt{ACT} command, a single row address controls a large-size \emph{logical} DRAM row, which spreads across all the mats in a subarray, and across all DRAM chips. A typical \SI{8}{\kilo\byte} size logical DRAM row is composed by addressing simultaneously 512 local bitlines in a mat across 16 mats in a DRAM subarray and 8 DRAM chips in a DRAM module (\SI{512}{\bit} per mat $\times$ 16 mats per chip $\times$ 8 chips per module = \SI{65536}{\bit} =  \SI{8}{\kilo\byte})~\cite{standard2012jesd79,seshadri2019dram,seshadri.bookchapter17,seshadri2017ambit,seshadri2016processing,zhang2014half}.
% During a \texttt{RD} command, the CSL selects a fraction (e.g., \SI{4}{\bit}) of data from each mat  using the column address, which is then transferred from the local row buffer to the global row buffer through the global bitlines. In a typical DDR4 DRAM  module~\cite{standard2012jesd79,seshadri2019dram,seshadri.bookchapter17,seshadri2017ambit,seshadri2016processing,zhang2014half}, a global row buffer logically latches \SI{64}{\byte} of the activated row, distributed across mats and chips (\SI{4}{\bit} per mat $\times$ 16 mats per chip $\times$ 8 chips per module = \SI{512}{\bit} = \SI{64}{\byte}).}
%
%++\gfbox{Atb: Aren't you only interested in coarse/fine grained activation? Why complicate with access if yes? ataberk too tired to edit now. Please remind him what the takeaway from this paragraph should be in the morning.}
Most commercial DRAM architectures employ a coarse-grained access and activation to exploit the temporal and spatial locality of an application's data access pattern. \gf{In this model, during an \texttt{ACT}, a single row address controls a large-size \emph{logical} DRAM row, which spreads across all the mats in a subarray, and across all DRAM chips.}
%\atb{ALTERNATIVE: In coarse-grained activation, an \texttt{ACT} command activates the local wordlines in \emph{all mats} in a subarray in every DRAM chip.}
%During DRAM access, the time taken to sense and latch a DRAM row dominates the total memory request time (the latency of an \texttt{ACT} command represents 71\% of the DRAM bank access time~\cite{Tiered-Latency_LEE}). By maintaining a large logical DRAM row containing several (e.g., 128) cache lines, DRAM can quickly service requests to consecutive cache lines (exploiting spatial locality) or repeated requests to the same cache line (exploiting spatial locality) from a previously-latched logical DRAM row. 
%However, DRAM's coarse-grained access and activation can lead to wasted energy consumption and throughput when an application does \emph{not} hold enough spatial and temporal locality.  
Many prior works~\cite{cooper2010fine,udipi2010rethinking,zhang2014half,ha2016improving,lee2017partial,olgun2022sectored} have investigated the issues caused by DRAM's coarse-grained access and activation in low-locality applications. To solve this issue, such works propose \emph{fine-grained} DRAM access and activation architectures. Their proposals are built based on the observation that DRAM's hierarchical organization \emph{already} provides a finer-grained activation granularity when considering the hardware structure of a single mat. 
%Thus, \gfi{they} focus on allowing individual control of a mat inside a DRAM array by partitioning the global wordline.
 }

\subsection{Processing-\gfcr{U}sing-DRAM}
\label{sec:background:pum}

\paratitle{In-DRAM-Row Copy} 
%RowClone~\cite{seshadri2013rowclone} is a mechanism that exploits the vast internal DRAM bandwidth to copy rows inside DRAM without CPU intervention efficiently.
RowClone~\cite{seshadri2013rowclone} enables copying a row~$A$ to a row~$B$ in the \emph{same} subarray by issuing two consecutive \texttt{ACT}
commands to these two rows, followed by a \texttt{PRE} command. This command sequence is called \texttt{AAP}~\omi{\cite{seshadri2017ambit}}.\revdel{ (\texttt{ACT}-\texttt{ACT}-\texttt{PRE})} \revdel{The first \texttt{ACT} copies the contents of the source row $A$ into the local row buffer. The second \texttt{ACT} connects the DRAM cells in the destination row~$B$ to the local bitlines. Because the sense amplifiers have already sensed and amplified the source data by the time row~$B$ is activated, the data in each cell of row~$B$ is overwritten by the data stored in the row buffer (i.e., row~$A$'s data). }%LISA~\cite{chang2016low} expands RowClone functionally to enable the execution of in-DRAM row copy operations across DRAM rows in \emph{different} subarrays of a DRAM chip
%by connecting local row buffers of neighbors subarrays 
%using isolation transistors.
%, enabling the execution of RowClone operations. 
%Recent works~\cite{gao2019computedram,olgun2022pidram} experimentally demonstrate the feasibility of executing in-DRAM row copy operations in unmodified off-the-shelf DRAM chips.

%\paratitle{In-DRAM Data Relocation} FIGARO~\cite{wang2020figaro} is a mechanism that enables data relocation in DRAM. It is built upon the key observation that the local row buffers inside a subarray in a bank are connected to a single shared global row buffer. FIGARO takes advantage of this connectivity to perform column-granularity data relocation across subarray without using the off-chip memory channel. To relocate data, FIGARO introduces a new DRAM command called \texttt{RELOC} (\emph{relocate column)}. The \texttt{RELOC} command moves a column $A$ (i.e., \SI{64}{\byte} data) stored in subarray $S_{A}$ to another column $B$ stored in subarray $S_{B}$ by:
%\li~activating the DRAM row that contains column $A$ in $S_{A}$, which latches the DRAM row to subarray $S_{A}$'s local row buffer;
%\lii~selecting column $A$ from subarray $S_{A}$'s local row buffer, which loads the column into the global row buffer; \liii~simultaneously connecting the global row buffer to subarray $S_{B}$ using subarray's $S_{B}$'s column decoder, which effectively places column $A$ from subarray $S_{A}$ into column $B$ of subarray $S_{B}$;
%\liv~activating subarray $S_{B}$, which overwrites column $B$ in the activated row with column $A$, since the global row buffer has a higher drive strength of the local row buffer~\cite{itoh2013vlsi,wang2020figaro}; and
%\lv~precharging the entire bank for future accesses. 


\paratitle{In-DRAM AND/OR/NOT}
Ambit~\ambit shows that simultaneously activating \emph{three} DRAM rows, via a DRAM operation called \emph{\gfi{\gls{TRA}}}, can perform \emph{in-DRAM} bitwise AND and OR operations.%When activating three rows, three cells connected to each local bitline share charge simultaneously and contribute to the perturbation of the local bitline.
\revdel{Upon sensing the perturbation \gf{of the three simultaneously activated rows}, the sense amplifier amplifies the local bitline voltage to $V_{DD}$ or 0 if at least two of the capacitors of the three DRAM cells are charged or discharged, respectively. As such, a \gfi{\gls{TRA}} results in a Boolean majority operation ($MAJ$).}
%A majority operation MAJ outputs a 1 (0) only if more than half of its inputs are 1 (0). %In terms of AND ($\cdot$) and OR (+) operations, a 3-input majority operation can be expressed as \texttt{MAJ(A, B, C) = A $\cdot$ B + A $\cdot$ C + B $\cdot$ C.} 
%
%To achieve functional completeness, Ambit implements NOT operations by exploiting the differential design of DRAM sense amplifiers. As Section~\ref{sec:background:dram} explains, the sense amplifier already generates the complement of the sensed value as part of the activation process. Therefore, Ambit simply forwards  the complement of the sensed value to a special DRAM row in the subarray that consists of DRAM cells with \emph{two} access transistors, called \emph{dual-contact cells} (DCCs). Each access transistor is connected to one side of the sense amplifier and is controlled by a separate wordline.% (\emph{d-wordline} or \emph{n-wordline}).
%By activating either the d-wordline or the n-wordline, the row of DCCs can provide the true or negated value stored in the row's cells, respectively.
%
%\rA{Ambit proposes \gfi{two} simple modifications to the DRAM array to \emph{efficiently} implement AND/OR/NOT operations. %\gfi{} internal organization of a subarray in Ambit, which has two different components than a conventional DRAM subarray. 
Ambit 
% Ambit implements MAJ by introducing a custom row decoder that can perform a TRA by simultaneously addressing three wordlines. To use this decoder, Ambit 
defines a new command called \texttt{AP} that issues a \gfi{\gls{TRA}}\revdel{ to compute a MAJ,} followed by a \texttt{PRE}\revdel{to close all three rows}.\revdel{\footnote{Although the `\texttt{A}' in \texttt{AP} refers to a \gls{TRA} operation instead of a conventional \texttt{ACT}, we use this terminology to remain consistent with the Ambit paper~\cite{seshadri2017ambit}, since an \texttt{ACT} can be internally translated to a TRA operation by the DRAM chip~\cite{seshadri2017ambit}.}} 
\rA{\changerA{\rA{\#A1}}Since TRA operations are destructive, Ambit divides DRAM rows into \emph{three groups} for \gls{PuD} computing: 
\li~the \textbf{D}ata group, which contains regular data rows;
\lii~the \textbf{C}ontrol group, which consists of two rows (\texttt{C0} and \texttt{C1})  with all-0 and all-1 values; and 
\liii~the \textbf{B}itwise group, which contains six rows designated for computation (four regular rows, \texttt{T0}, \texttt{T1}, \texttt{T2}, \texttt{T3}; and two rows, \texttt{DCC0} and \texttt{DCC1},  of dual-contact cells {for NOT)}.
%The D-group contains regular rows that store program or system data. The C-group consists of two constant rows, called C0 and C1, that contain all-0 and all-1 values, respectively, used to control the execution of AND (C0 row) and OR (C1 row) operations. The D-group and the C-group are connected to the regular local row decoder, which selects a single row at a time. The B-group contains six regular rows %, called T0, T1, T2, and T3; 
%and two rows of dual-contact cells%, 
%whose d-wordlines are called DCC0 and DCC1, and whose n-wordlines are called $\overline{\mbox{DCC0}}$ and $\overline{\mbox{DCC1}}$, respectively
\revdel{The B-group rows are designated to perform bitwise operations. They are all connected to a special local row decoder that can simultaneously activate three rows using a single address 
(i.e., perform a \gfi{\gls{TRA}}).}
%Using a typical subarray size of 1024 rows~\cite{chang2014improving, kim2012case, kim2018solar,Tiered-Latency_LEE,kim2019d}, Ambit splits the row addressing into 1006 D-group row addresses, 2 C-group row addresses, and 16 B-group rows addresses.
}


% \begin{figure}[ht]
%     %\vspace{-5pt}
%     \centering
%     \includegraphics[width=\linewidth]{figures/ambit_subarray-crop.pdf}
%     \caption{Ambit's subarray organization.}
%     \label{fig_subarray_ambit}
%    % \vspace{-10pt}
% \end{figure}

\paratitle{Generalizing In-DRAM Majority} SIMDRAM~\cite{hajinazarsimdram} \omiii{proposes} a three-step framework to implement \gfi{\gls{PuD}} operations. In the first step, SIMDRAM converts an AND/OR/NOT-based representation of the desired operation into an equivalent optimized MAJ/NOT-based representation. \rA{\changerA{\rA{\#A1}}By doing so, SIMDRAM reduces the number of TRA operations required to implement the operation.} 
In the second step, SIMDRAM generates the required sequence of DRAM commands to execute the desired operation. \rA{\changerA{\rA{\#A1}}Specifically, this step translates the MAJ/NOT-based implementation of the operation into \texttt{AAPs}/\texttt{APs}.
This step involves \li~allocating the designated compute rows in DRAM to the operands and \lii~determining the optimized sequence of \texttt{AAPs}/\texttt{APs} that are required to perform the operation.} 
This step's output is a \uprog, i.e., the optimized sequence of \texttt{AAPs}/\texttt{APs} that will be used to execute the operation at runtime. \gfcrii{Each \uprog corresponds to a different \emph{bbop} instruction, which is one of the CPU ISA extensions to allow programs to interact with the SIMDRAM framework (see \cref{sec:design:isa}).} 
In the third step, SIMDRAM uses a control unit in the memory controller to \omi{execute the \emph{bbop} instruction using the corresponding} \uprog. 
%SIMDRAM uses a control unit in the memory controller that transparently issues the sequence of \texttt{AAPs}/\texttt{APs} to DRAM, as dictated by a \emph{bbop} instructions. %Once a \emph{bbop} instruction is complete, the result of the in-DRAM computation is held in DRAM. 
\rA{{SIMDRAM implements} 16 \emph{bbop} instructions, including abs, add, bitcount, div, max, min, mult, ReLU, sub, and-/or-/xor-reduction, equal, greater, greater equal, and if-else.} 
%

\rA{\changerA{\rA{\#A1}}Fig.~\ref{fig:simdram:example} illustrates how SIMDRAM executes a \gfcrii{one}-bit full addition operation using the sequence of row copy (\texttt{AAP}) and majority (\texttt{AP}) operations in DRAM. The figure shows one iteration of the full adder computation that computes \texttt{Y$_{0}$ = A$_{0}$ + B$_{0}$ + C$_{in}$}. 
First, }\gfi{SIMDRAM uses a \emph{vertical} data layout, where all bits of a \gfcrii{data element} are placed in a single DRAM column\revdel{ (i.e., in a single bitline),} when performing \gfi{PuD} computation.} 
%By doing, SIMDRAM can execute bit-shift operations, which is essential \gfi{in} complex computations without extra area cost. 
%For example, SIMDRAM can perform a left-shift-by-one operation by copying (using RowClone) the data in DRAM row $j$ to DRAM row $j+1$. 
Consequently, SIMDRAM employs a \emph{bulk bit-serial \gls{SIMD}} execution model, where each \gfcrii{data element} is mapped to a column of a DRAM row. This allows a DRAM subarray to operate as a \emph{\gfi{PuD} SIMD engine}, where a single bit-serial operation is performed over a large number of independent \gfcrii{data elements} \omii{(i.e., as many \gfcrii{data elements} as the size of a logical DRAM row, for example, 65,536)} at once. \rA{Second, as shown in the figure, each iteration of the full adder requires five \texttt{AAP}s \gfcrii{(\circled{1}, \circled{2}, \circled{3}, \circled{6}, \circled{7}) and three \texttt{AP}s (\circledgreen{4}, \circledgreen{5}, \circledgreen{8})}. 
A bit-serial addition of $n$-bit operands needs $n$ iterations, thus $(8 × n + 2)$ \texttt{AP}s \omii{and} \texttt{AAP}s~\omii{\cite{hajinazarsimdram}}.
}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/example_addition-crop.pdf}%
    %\vspace{-8pt}
    \caption{\gfcriii{Full adder operation in SIMDRAM.}}
    \label{fig:simdram:example}
\end{figure}


% To enable a fast conversion between horizontally-layout data (used by the CPU) and vertically-layout data (used by \emph{bbop} instructions), SIMDRAM implements a data \emph{transposition unit} placed between the last-level cache and the memory controller. The transposition unit tracks data structures that are consumed/produced by a \emph{bbop} instruction (manually identified by the programmer). It automatically transposes such data structures' cache lines from a horizontal to vertical data layout (during cache evictions) and from a vertical to horizontal data layout (during cache line reads from main memory).     



%\paratitle{In-DRAM Look-Up Tables} 

%\paratitle{Alternative Processing-using-DRAM Architectures}




==> mainmatter/05_mimdram/sections/07_related_work.tex <==
\section{Related Work}
\label{sec:related}

To our knowledge, \prop is the first \omi{end-to-end processing-using-DRAM (\gls{PuD})} system \gfcrii{for general-purpose applications that executes operations in a multiple-instruction multiple-data (MIMD) fashion, where \emph{independent} \gls{PuD} operations are executed \emph{concurrently} across the DRAM mats of a DRAM subarray.}  We highlight \prop's key contributions by contrasting it with state-of-the-art processing-in-memory \gfcrii{(PIM)} designs. \omi{We already compared \prop to SIMDRAM~\cite{hajinazarsimdram}, DRISA~\cite{li2017drisa}, and Fulcrum~\cite{lenjani2020fulcrum} both \emph{quantitatively} and \emph{qualitatively} in \cref{sec:eval} and demonstrated \prop's benefits over them. } 


\revdel{\paratitle{Fine-Grained DRAM} Several prior works~\cite{lee2017partial,zhang2014half,zhang2017enabling,alawneh2021dynamic,son2014microbank,oconnor2017fine,chatterjee2017architecting,cooper2010fine,ha2016improving,udipi2010rethinking} propose different mechanisms to enable fine-grained DRAM substrates, aiming to alleviate the energy waste caused by coarse-grained DRAM. 
%These works achieve fine-grained DRAM activation and access using varying approaches (e.g., reorganizing the DRAM array and/or modifying the DRAM on-chip interconnect; adding more HFFs~\cite{zhang2017enabling,alawneh2021dynamic,son2014microbank,oconnor2017fine,chatterjee2017architecting}). 
\prop builds on top of such works to enable fine-grained DRAM activation for \gls{PuD} computing. 
Another class of prior work~\cite{yoon2011adaptive,yoon2012dynamic,ahn2009multicore,zheng2008minirank,brewer2010instruction} proposes new DRAM module designs that allow independently operating each DRAM chip in a DRAM module to implement fine-grained DRAM access. The concepts \prop introduces are orthogonal to such works, and can be combined with fine-grained DRAM access.}

\paratitle{Processing-\gfcr{U}sing-DRAM} 
Prior works propose different ways of implementing \gls{PuD} operations, either by 
\li~using the memory arrays themselves to perform  operations in bulk~\cite{seshadri.bookchapter17, seshadri2013rowclone,seshadri2018rowclone,wang2020figaro,seshadri2017ambit, xin2020elp2im, besta2021sisa,deng2018dracc, gao2019computedram,li2017drisa, hajinazarsimdram,li2018scope,ferreira2021pluto,ferreira2022pluto,deng2019lacc,olgun2021quactrng,bostanci2022dr} \omi{or}
\lii~modifying the DRAM sense amplifier design with logic gates for computation~\cite{li2017drisa,zhou2022flexidram}. 
\revdel{\gfcrii{\prop provides two main benefits \omii{over} these \gls{PuD} architectures.}} 
\gfcrii{Since} prior \gls{PuD} architectures execute \gls{PuD} operations at a \omii{coarse} granularity (i.e., at the granularity of a DRAM row access), they can suffer from the \underutilization issue we highlight. 
As in \prop, prior \gls{PuD} architectures can employ fine-grained DRAM for \gls{PuD} operations to mitigate \underutilization.
\gfcriii{We believe that the principles employed in \prop\revdel{, both in hardware and in software,} can benefit other \gls{PuD} architectures, leading to performance\omiii{,} energy-\omiii{efficiency}\omiii{, and programmability} improvements for the underlying \gls{PuD} substrate.}

\paratitle{Programming Support for \gls{PuM}} 
Prior works propose programming models for different types of \gls{PuM} architectures, as
\li~CUDA/OpenAcc~\cite{cheng2014professional, OpenACCA1:online} for in-cache computing~\cite{dualitycache};
\lii~tensor dataflow graphs for \revdel{in-cache~\cite{wang2023infinity} and }in-ReRAM computing~\cite{fujiki2018memory}. By enabling fine-grained DRAM, we believe such programming models can be \omi{now easily} ported to \gfi{\gls{PuD}} computing (for example, by assuming that each DRAM mat executes a different CUDA thread block).  
CHOPPER~\cite{peng2023chopper} improves SIMDRAM's programming model by leveraging bit-slicing compilers and employing optimizations to reduce the latency of a \uprog. Even though CHOPPER simplifies \omiii{programmability} compared to SIMDRAM, it still requires the programmer to re-write applications using the bit-slicing compiler's syntax. Compared to CHOPPER, \prop has two main advantages. First, \prop \emph{automatically} generates code for the \gfi{\gls{PuD}} engine without any code refactoring. Second, since CHOPPER maintains the \gfcrii{very}-wide \gls{SIMD} programming model of SIMDRAM, it \omi{also} suffers from  \gls{SIMD} underutilization.


==> mainmatter/06_proteus/macros_proteus_old.tex <==
% Mechanism Name
\renewcommand{\prop}{\emph{Proteus}\xspace}

% PUD-related macros
\providecommand\bbop{\emph{bbop}\xspace}
\providecommand\uproglib{\emph{parallelism-aware \uprog library}\xspace}
\providecommand\dynengine{\emph{dynamic bit-precision engine}\xspace}
\providecommand\uprogunit{\emph{\uprog select unit}\xspace}
\providecommand\bitprec{\emph{bit-precision calculator unit}\xspace}
\providecommand\objtrack{\emph{object tracker}\xspace}
\providecommand\costmodel{\emph{cost model logic}\xspace}
\providecommand\gbidx{\emph{global\_\textmu{}Program\_idx}\xspace}
\providecommand\idx{\emph{\textmu{}Program\_idx}\xspace}
\providecommand\aap{\texttt{AAP}/\texttt{AP}\xspace}
\providecommand\aaps{\texttt{AAP}s/\texttt{AP}s\xspace}
\providecommand\uop{\textmu{}Op\xspace}
\providecommand\uops{\textmu{}Ops\xspace}
\providecommand\uprog{\textmu{}Program\xspace}
\providecommand\uprogs{\textmu{}Programs\xspace}

% Text editing
\providecommand\ignore[1]{ }
\providecommand{\sgdel}[1]{}

% Paper Submission Macros
\newif\ifasplosrevisionsubmission
\asplosrevisionsubmissiontrue
%\asplosrevisionsubmissionfalse
\ifasplosrevisionsubmission
    \providecommand{\omrev}[1]{#1}
\else
    \providecommand{\omrev}[1]{\textcolor{orange}{#1}}
\fi

\newif\ifproteusasplosrevision
%\proteusasplosrevisiontrue
\proteusasplosrevisionfalse
\ifproteusasplosrevision 
    \providecommand{\asplosrev}[1]{\textcolor{blue}{#1}}
\else
    \providecommand{\asplosrev}[1]{\textcolor{black}{#1}}
    \renewcommand{\hl}[1]{#1}
\fi

\newif\ifproteusasplossubmission
\proteusasplossubmissiontrue
%\proteusasplossubmissionfalse
\ifproteusasplossubmission 
    \providecommand{\gfasplos}[1]{\textcolor{black}{#1}}
    \providecommand{\agyasplos}[1]{\textcolor{black}{#1}}
    %\newcommand{\param}[1]{#1}
    \providecommand{\agyasploscomment}[1]{}
\else
    \providecommand{\gfasplos}[1]{\textcolor{blue}{#1}}
    %\newcommand{\param}[1]{\textcolor{red}{#1}}
    \providecommand{\agyasplos}[1]{\textcolor{red}{#1}}
    \providecommand{\agyasploscomment}[1]{\textcolor{red}{\textbf{!!!~Giray:} #1}}
    
\fi

\newif\ifproteusmicrosubmission
\proteusmicrosubmissiontrue
%\proteusmicrosubmissionfalse
\ifproteusmicrosubmission 
    \providecommand{\gfmicro}[1]{\textcolor{black}{#1}}
    \providecommand{\agymicro}[1]{\textcolor{black}{#1}}
    \providecommand{\param}[1]{#1}
    \providecommand{\agymicrocomment}[1]{}
\else
    \providecommand{\gfmicro}[1]{\textcolor{blue}{#1}}
    \providecommand{\param}[1]{\textcolor{red}{#1}}
    \providecommand{\agymicro}[1]{\textcolor{red}{#1}}
    \providecommand{\agymicrocomment}[1]{\textcolor{red}{\textbf{!!!~Giray:} #1}}
    
\fi

\newif\ifproteusiscarevision
%\proteusiscarevisiontrue
\proteusiscarevisionfalse
\ifproteusiscarevision 
    \providecommand{\revA}[1]{\textcolor{red}{#1}}
    \providecommand{\revB}[1]{\textcolor{mygreen}{#1}}
    \providecommand{\revC}[1]{\textcolor{safetyorange}{#1}}
    \providecommand{\revD}[1]{\textcolor{heliotrope}{#1}}
    \providecommand{\revE}[1]{\textcolor{rufous}{#1}}
    \providecommand{\revCommon}[1]{\textcolor{blue}{#1}}

    % \providecommand{\changeCM}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1,size=\scriptsize]{\revCommon{\textbf{#2}}}}
    
    % \newcommandx{\changeA}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1,size=\scriptsize]{\revA{\textbf{#2}}}}
    
    % \newcommandx{\changeB}[2][1=]{\todo[linecolor=mygreen,backgroundcolor=mygreen!25,bordercolor=mygreen,#1,size=\scriptsize]{\revB{\textbf{#2}}}}
    
    % \newcommandx{\changeC}[2][1=]{\todo[linecolor=safetyorange,backgroundcolor=safetyorange!25,bordercolor=safetyorange,#1,size=\scriptsize]{\revC{\textbf{#2}}}}
    
    % \newcommandx{\changeD}[2][1=]{\todo[linecolor=heliotrope,backgroundcolor=heliotrope!25,bordercolor=heliotrope,#1,size=\scriptsize]{\revD{\textbf{#2}}}}
    
    % \newcommandx{\changeE}[2][1=]{\todo[linecolor=rufous,backgroundcolor=rufous!25,bordercolor=rufous,#1,size=\scriptsize]{\revE{\textbf{#2}}}}
\else
    \providecommand{\revA}[1]{\textcolor{black}{#1}}
    \providecommand{\revB}[1]{\textcolor{black}{#1}}
    \providecommand{\revC}[1]{\textcolor{black}{#1}}
    \providecommand{\revD}[1]{\textcolor{black}{#1}}
    \providecommand{\revE}[1]{\textcolor{black}{#1}}
    \providecommand{\revCommon}[1]{\textcolor{black}{#1}}

    \providecommand{\changeCM}[2][1=]{\todo[disable,#1]{#2}}
    \providecommand{\changeA}[2][1=]{\todo[disable,#1]{#2}}
    \providecommand{\changeB}[2][1=]{\todo[disable,#1]{#2}}
    \providecommand{\changeC}[2][1=]{\todo[disable,#1]{#2}}
    \providecommand{\changeD}[2][1=]{\todo[disable,#1]{#2}}
    \providecommand{\changeE}[2][1=]{\todo[disable,#1]{#2}}
\fi

\newif\ifcut
%\cuttrue
\cutfalse
\ifcut
   \providecommand{\gfcut}[1]{} 
\else
    \providecommand{\gfcut}[1]{\textcolor{red}{\sout{#1}}}
\fi 


\newif\ifproteusiscasubmission
\proteusiscasubmissiontrue
%\proteusiscasubmissionfalse
\ifproteusiscasubmission
    \providecommand{\gfisca}[1]{#1}
    \providecommand{\gfbisca}[1]{}
    \providecommand{\sg}[1]{#1}
    \providecommand{\sgi}[1]{#1}
    \providecommand{\om}[1]{#1}
\else
    \providecommand{\gfbisca}[1]{\textcolor{blue}{\textit{GF: #1}}}
    \providecommand{\gfisca}[1]{\textcolor{blue}{#1}}

    \providecommand{\sg}[1]{\textcolor{red}{#1}}
    \providecommand{\sgi}[1]{\textcolor{brickred}{#1}}

    \providecommand{\om}[1]{\textcolor{orange}{#1}}
\fi


\newif\ifproteussubmission
\proteussubmissiontrue
%\proteussubmissionfalse
\ifproteussubmission
    \providecommand{\kangqi}[1]{#1}
    \providecommand{\juan}[1]{#1}
    \providecommand{\gf}[1]{#1}
    \providecommand{\gfii}[1]{#1}
    
    \providecommand{\jgl}[1]{}

    \providecommand{\gfb}[1]{}
    %\newcommand{todo}[1]{#1}
    \providecommand{\mayank}[1]{}
    \providecommand{\ms}[1]{#1}
    \providecommand{\agy}[1]{#1}
    \providecommand{\agycomment}[1]{}
\else
    \providecommand{\jgl}[1]{\textcolor{brickred}{\textit{JGL: #1}}}
    \providecommand{\gfb}[1]{\textcolor{blue}{\textit{GF: #1}}}
    \providecommand{\todo}[1]{\textcolor{red}{\textbf{TODO: #1}}}
    \providecommand{\juan}[1]{\textcolor{brickred}{#1}}
    \providecommand{\mayank}[1]{\textcolor{green}{\textit{Mayank: #1}}}
    \providecommand{\kangqi}[1]{\textcolor{byzantium}{#1}}
    \providecommand{\gf}[1]{\textcolor{blue}{#1}}

    \providecommand{\gfii}[1]{\textcolor{red}{#1}}
    
    \providecommand{\ms}[1]{\textcolor{cyan}{#1}}
    \providecommand{\agy}[1]{\textcolor{orange}{#1}}
    \providecommand{\agycomment}[1]{\agy{\textbf{[@gy:} #1\textbf{]}}}

\fi



==> mainmatter/06_proteus/packages_proteus.tex <==
\PassOptionsToPackage{hyphens}{url}
\usepackage[bookmarks=true,breaklinks=true,colorlinks,linkcolor=black,citecolor=black,urlcolor=blue]{hyperref}

\usepackage[normalem]{ulem}
%\usepackage{multirow}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%\usepackage{stmaryrd}
%\usepackage{amsmath}
%\usepackage{listings}
\usepackage{subcaption}
\usepackage{clipboard}
\usepackage{soul}
%\usepackage[super]{nth}
\usepackage{tikz}
\usepackage{flushend}
%\usepackage[table,xcdraw]{xcolor}
\usepackage[noadjust]{cite}
\usepackage{xargs} 
%\usepackage{todonotes}
%\usepackage[binary-units=true]{siunitx}
%\usepackage{tikzducks}
%\usepackage{duckuments}
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage{booktabs}
%\usepackage{multirow}
%\usepackage{siunitx}
\usepackage[many]{tcolorbox}% version 2.80 (2014/03/31)
\usepackage{longfbox}

%\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{pifont}
\usepackage[acronym,nonumberlist,nowarn]{glossaries}
    \glsdisablehyper
     \loadglsentries{support/acronyms}


\usepackage{xspace}
\usepackage[binary-units=true]{siunitx}
\usepackage{todonotes}

\usepackage{balance}


%\newcommand{\subparagraph}{}

%\usepackage[explicit]{titlesec}
\usepackage{setspace}
\usepackage[export]{adjustbox}

\usepackage{fancyhdr}
%\usepackage[hyphens]{url}


\usepackage{cleveref}
\crefformat{section}{\S#2#1#3}
\crefformat{subsection}{\S#2#1#3}
\crefformat{subsubsection}{\S#2#1#3}

%\usepackage{hyperref}

%\hypersetup{
%  colorlinks   = true, %Colours links instead of ugly boxes
%  urlcolor     = blue, %Colour for external hyperlinks
%  linkcolor    = blue, %Colour of internal links
%  citecolor   = black %Colour of citations
% }


==> mainmatter/06_proteus/sections/00_abstract.tex <==
\begin{abstract}
% \vspace{1pt}
% 
\Gls{PuD} is \om{a paradigm where the analog operational properties of DRAM structures are used to perform \sgi{bulk} logic operations.}
\revdel{PIM trend that proposes to compute using the analog operation of DRAM cells.}%
\sgdel{Due to DRAM's \om{large} internal parallelism, }%
\sgi{While} \gls{PuD} promises high throughput at low energy and area cost,
% \om{Unfortunately}, 
\sgi{we uncover three limitations of existing \gls{PuD} approaches that lead to significant inefficiencies:} 
\li~static data representation\om{, i.e., 2's complement \sgdel{data representation}%
 with fixed bit-precision, leading to \emph{unnecessary computation} over useless \asplosrev{\hl{(i.e., inconsequential)}} data}; 
\lii~support for \emph{only} throughput-oriented execution\om{, where the high latency of individual \gls{PuD} operations can \emph{only} be hidden in the presence of bulk data-level parallelism;} and 
\liii~high latency for high-precision \om{(e.g., 32-bit) operations}. 
%
\sgi{To address these issues, we propose \prop,}
\sgdel{To address these issues, we propose \prop, an adaptive \emph{data-representation} and \emph{operation-implementation} framework.}%
\om{which builds on two \emph{key ideas}. 
First, \prop \emph{parallelizes} the execution of independent primitives in a \gls{PuD} operation by leveraging DRAM's internal parallelism. 
Second, \prop \emph{reduces} the bit-precision for \gls{PuD} operations by leveraging \emph{narrow values} (i.e., values with many leading zeros).}
\revdel{\sgi{We design an adaptive framework for \prop that uses hardware support at runtime, \emph{transparent} from the user, to select}
% \om{Based on these two key ideas, we design \prop as a three-components hardware framework for high-performance \gls{PuD} computation that \emph{transparently} from the user selects} 
\li~the most efficient data format (e.g., 2's complement, redundant binary), 
\lii~the exact \sgi{bit-precision for a workload}, and
\sgdel{data precision that a workload requires (e.g., non-power-of-two integers), and}%
\liii~the fastest algorithm (e.g., bit-serial, bit-parallel) for latency- or throughput-oriented execution. }
%
%\prop builds upon prior works that enhance DRAM to perform intra-subarray/inter-subarray data movement, bulk bitwise operations, and subarray-level parallelism. 
% \jgl{We may want to mention more key ideas here?} 
% \kangqi{To accommodate a wider range of arithmetic operations and real-world kernels, \prop{} further includes enhancement such as an upgraded inter-bank data movement mechanism and a Near-Bank Shifter for the ease of data manipulation, and an in-DRAM wrap-around data mapping for the throttling of computation resource usage. }
%algorithm that explores different data representations such as 2's complement and redundant binary and bit serial and bit-parallel algorithms. 
% Additionally, the research uses DRAM enhancements proposed in prior work, such as LISA, SALP, and FIGARO, to improve system performance.
%
\gf{We compare \prop to different state-of-the-art computing platforms (CPU, GPU, and the SIMDRAM \gls{PuD} architecture) \gfisca{for \om {twelve} real-world applications.} 
Using a single DRAM bank, 
\gfisca{\prop provides 
\li~17$\times$, 7.3$\times$, and 10.2$\times$ the performance per mm$^2$; and
\lii~90.3$\times$, 21$\times$, and 8.1$\times$ \om{lower energy consumption than that} of the CPU, GPU, and SIMDRAM, respectively, on average across \om{twelve} real-world applications.
\prop incurs low area cost on top of a DRAM chip (1.6\%) and CPU die (0.03\%).}}

% \juan{As a result, %\prop{}
% \ms{\prop} outperforms the state-of-the-art processing-using-DRAM approach.} 
% % \jgl{We need a summary of results for microbenchmarks, benchmarks, and comparison to CPU, GPU, and SIMDRAM.}
% \kangqi{We demonstrate the superiority of %\prop{} 
% \ms{\prop} over CPU, GPU, and the state-of-the-art processing-using-DRAM approach, SIMDRAM, through micro-benchmarks like GEMV and real-world kernels like Neural Networks. Based on our evaluation, \ms{\prop}%\prop{} 
% outperforms the SIMDRAM baseline by (1) 1.5-12$\times$ and 1.2-6$\times$ for Vector Addition and Multiplication, respectively; (2) 1-15$\times$ and 1-2$\times$ for reduction and GEMV kernel. In terms of Neural Networks, %\prop{} 
% \ms{\prop} is also capable of delivering maximally 2$\times$ performance and 8$\times$ power reduction over a high-end GPU. Nevertheless, \prop{} incurs a 2.5\% area overhead per DRAM bank}. 

%\jgl{Do we need the next two paragraphs? Likely not.}
%The proposed system includes an emulator\mayank{Should it be a compiler or simulator or what ?} \prop{} that creates an adaptive algorithm based on different data representation and algorithm approaches, which can improve the accuracy of calculations while maximizing the resource utilization and enable parallelism. These features optimize system performance and efficiency in latency, energy, and throughput by efficiently using available resources.

%Overall, this research presents a promising direction for improving the performance and efficiency of computing systems by using and characterizing PIM architectures based on any DRAM substrate (DDR, HBM, etc.). By taking advantage of memory enhancements and introducing adaptive algorithms, the proposed system can overcome the limitations of existing processing-using-DRAM approaches and improve system performance. We aim to open source \prop{} on GitHub.  
%\mayank{write results}
%\mayank{Should we compare this w.r.t AREA also from other works like fulcrum, DRISA, etc. ?}
%\mayank{should we talk about inline assembly that will be generated because some new instructions will be introduced?}

% Evaluation of different DRAM types (with varying subarray sizes, row buffer sizes, timing intervals...).

% Comparison to CPU, GPU, SIMDRAM \& other PuDRAM (e.g., horizontal layout), PNM (UPMEM).


\end{abstract}

==> mainmatter/06_proteus/sections/01_introduction.tex <==
\glsresetall

\section{Introduction}
\label{sec:introduction}

\gf{\Gls{PIM}~\pimdef 
\sgdel{is a promising paradigm that}%
aims to alleviate the ever-growing cost of moving data\revdel{ back-and-forth} \juan{between} computing (e.g., CPU, GPU) and memory (e.g., DRAM) elements. In \gls{PIM} architectures, computation is done by adding logic \emph{near} memory arrays, i.e., \gls{PnM}~\pnm, or by \emph{using} the analog properties of the memory arrays, i.e., \gls{PuM}~\pum). 
Many prior works~\drampum  demonstrate the %ability to implement 
\juan{feasibility of} \gls{PuD}, which use DRAM cells to implement \gfasplos{in-DRAM row copy~\cite{seshadri2013rowclone,seshadri2018rowclone,gao2019computedram}, Boolean~\cite{li2017drisa,seshadri2017ambit,xin2020elp2im}, and arithmetic~\cite{hajinazarsimdram,deng2018dracc,angizi2019graphide,li2018scope,peng2023chopper,mimdramextended} operations.}\revdel{ a variety of \gls{PuM} operations\revdel{, including bitwise Boolean~\cite{seshadri2017ambit, gao2019computedram, xin2020elp2im, besta2021sisa, li2017drisa} and arithmetic operations~\cite{deng2018dracc, gao2019computedram,li2017drisa,angizi2019graphide, hajinazarsimdram,li2018scope}}.}} 
%
\gf{\revdel{\gls{PuD} architectures leverage the key observations that 
\li~DRAM can perform Boolean \sgi{primitives} (e.g., NOR, MAJ) by simultaneously accessing (i.e., activating) multiple \sgdel{(e.g., three)}%
DRAM rows, and
\lii~complex arithmetic operations (e.g., addition) can be built by composing sequences of Boolean \sgi{primitives}.} 
\revdel{\sgi{\gls{PuD} frameworks~\cite{hajinazarsimdram, peng2023chopper} automate the implementation of complex arithmetic} operations using in-DRAM Boolean operations.} 
\sgi{\gfmicro{\gls{PuD} systems often} employ a \emph{bulk bit-serial} execution model, where each Boolean primitive operates across entire DRAM rows, with each row containing one bit from many input operands.
The predefined sequence of DRAM commands used to implement each operation are stored in a \emph{\uprog}.}
\sgdel{Such frameworks employ a  \emph{bulk bit-serial} execution model. In this execution model, a \gls{PuD} operation is performed by \emph{sequentially} activating different DRAM rows, each of which stores one bit from the input operand, one row (i.e., a bit from the input operand) per time, following a predefined sequence of DRAM commands (called a \emph{\uprog}). 
Thus, the number of bits used to represent operands (i.e., the \emph{bit-precision}) directly impacts the latency of a \gls{PuD} operation.
\sgi{Existing \gls{PuD} architectures employ a fixed-width bit representation to simplify execution.}}}
%\gf{For example, the latency of executing \gls{PuD} addition and multiplication operations scales linearly and quadratically with the bit-precision of the input operands~\cite{hajinazarsimdram,peng2023chopper}.}
%\jgl{May be good to mention examples as linear dependency for addition and quadratic for multiplication.}

\sgi{\revdel{Unfortunately, while prior works have demonstrated the benefits of \gls{PuD} for several applications~\cite{seshadri2017ambit, xin2020elp2im, besta2021sisa,deng2018dracc, gao2019computedram,li2017drisa,angizi2019graphide, hajinazarsimdram,li2018scope},}
\gfasplos{In this work,} we uncover three limitations that significantly hurt the performance and efficiency of \gls{PuD} architectures.
First, they employ a \emph{static bit-precision} \gfmicro{for operands} (i.e., the number of bits used to represent an operand), which is wider than the maximum data values being computed on.
This results in significant wasted latency and energy to perform calculations on inconsequential bits (e.g., \asplosrev{\hl{leading zeros in case of positive numbers or leading ones in case of negative numbers}}).
Second, they aim to \emph{maximize execution throughput} for large data sets, \gfasplos{to} overcome long bit-serial latencies and take advantage of the large amount of in-DRAM parallelism.
Whenever these architectures execute on smaller data sets, much of this parallelism \asplosrev{\hl{is not fully utilized}},
\emph{even though there are opportunities to better exploit this parallelism to improve latency and efficiency.}
Third, they suffer from \emph{high latencies for high-precision computation} due to their bit serialization.
\revdel{Forcing bit-serial computation instead of leveraging alternate execution models can significantly harm program efficiency.}
Ultimately, these limitations exist because there is no one-size-fits-all solution for data representation and execution model across a wide range of applications.}

\sgdel{\gf{Even though prior works have demonstrated the performance and energy benefits of employing \gls{PuD} for several applications, they suffer from \emph{three} main limitations caused by naively using a bit-serial execution model, which in turn,  hinder their performance. 
First, they \emph{undermine} the full benefits of the underlying bit-serial execution model by using a \emph{static data representation} for \gls{PuD} computation. 
This is because prior works utilize conventional data formats (e.g., 2's complement) and operands' bit-precision (e.g., 32-bit integers) for \gls{PuD} computation even when computation could be performed with fewer bits, leading to subpar performance.
Second, they \emph{only} support a \emph{throughput-oriented execution}, which can hurt the overall performance of latency-sensitive operations. \gls{PuD} architecture often favors throughput-oriented execution because the bulk parallelism inside a DRAM array can %hide 
\juan{amortize} the latency of consecutive DRAM activations in a \uprog. 
\revdel{To break even in terms of performance (compared to a processor-centric execution), the \gls{PuD} operation needs to operate over large input sets to fully utilize the bulk parallelism the underlying \gls{PuD} architecture offers.} When executing \gls{PuD} operations with smaller-than-ideal input set sizes \juan{(e.g., less than the DRAM row size)}, the \gls{PuD} architecture can experience sub-optimal performance or even performance loss compared to their processor-centric counterparts.    
Third, they suffer from \emph{high latency} when executing \emph{high-precision computation}. In a bit-serial execution model, the computation latency scales with bit-precision used for operands. This scaling can \emph{significantly} degrade performance when using a large bit-precision (e.g., 64-bits) for quadratically-scaling bit-serial \gls{PuD} operations \gfisca{(e.g., multiplication, division)}.}}

\gf{Our \emph{goal} in this work is to overcome the three limitations of \gls{PuD} architectures caused by naively employing a bit-serial execution model. To this end, we propose \prop,\footnote{\gfasplos{\prop is a shape-shifting, prophetic sea god from Greek mythology, known for his ability to elude capture by changing forms.} As such, \prop \emph{changes} the bit-precision of \gls{PuD} operations to improve performance.} an efficient \gls{PuD} framework with \gfisca{adaptive} bit-precision \gfisca{and dynamic arithmetic}. The \emph{key ideas} behind \prop are: 
\li~fully leverage the parallelism \sgi{within} a DRAM bank to accelerate the execution of various bit-serial and bit-parallel arithmetic operations, and 
\lii~decide \sgi{at runtime} the best-performing bit-precision, data representation format, and algorithmic implementation of \sgi{each \gls{PuD}} operation. \prop is composed of three main components: \uproglib, \dynengine, and \uprogunit. \revdel{With these three components, \prop can adapt the data representation and \gls{PuD} operation implementation depending on the target bit-precision.}}

\gf{First, we build a  \uproglib, which consists of hand-tuned implementations of key arithmetic operations using various bit-serial and bit-parallel algorithms and data representation formats. 
To improve the\gfmicro{ir } performance, we \revdel{fully leverage the parallelism available inside a DRAM bank (i.e., subarray-level parallelism~\cite{kim2012case}). 
Concretely, we} carefully craft 
%\jgl{craft? Present sounds better.} 
different implementations of a given \gls{PuD} operation to parallelize the execution of \gfmicro{independent} steps in a \uprog across different DRAM subarrays\revdel{, in what we refer to as \emph{one-bit per-subarray (OBPS)} method}. %OBPS is enabled by \juan{leveraging} prior works that allow %s
%\li~the activation of different DRAM subarrays concurrently (i.e., SALP~\cite{kim2012case}) and
%\lii~moving data across DRAM subarrays efficiently (i.e., LISA~\cite{chang2016low}). 
Our \emph{parallelism-aware \uprog library} considers different data representation formats that can be %better 
\juan{more} suitable for high-precision arithmetic. 
Namely, we implement variations of our algorithms using both 2's complement and \gls{RBR}~\cite{guest1980truth,phatak1994hybrid,lapointe1993systematic}. Unlike binary numeral systems,\revdel{ which use a single bit to represent an operand,} \gls{RBR} uses a pair of bits to represent an operand. This allows \gls{RBR}-based arithmetic to be performed \emph{without} the need for long \gfasplos{and costly} carry propagation chains\revdel{, which can be a costly during \gls{PuD} execution}. In the end, the \emph{parallelism-aware \uprog library} contains a collection of possible implementations of desired \gls{PuD} operations, each of which with different time complexities that depend on the target bit-precision. 
%
Second, we devise a new \dynengine to identify the appropriate initial bit-precision for a given \gls{PuD} operation. We implement the  \dynengine by augmenting prior works' data transposition engine\juan{~\cite{hajinazarsimdram,mimdramextended}}. Before \gls{PuD} execution,  the data transposition engine captures and transposes (from the standard horizontal data layout to the \gls{PuD} vertical data layout) cache lines that are about to be evicted from the \gls{LLC}  to DRAM and belong to a previously-identified \gls{PuD} memory object. During this process, our  \dynengine \emph{\gfmicro{scans}} the content of the evicted cache line to identify the largest value belonging to \gfasplos{a} \gls{PuD} memory object.\revdel{ Based on this value, the \dynengine sets the most appropriate bit-precision when the \gls{PuD} operation needs to be executed.} 
Third, when the user issues a \gls{PuD} operation, the \uprogunit probes the \dynengine to identify the most suitable bit-precision for the \revdel{incoming }\gls{PuD} operation and\revdel{ based on an analytical cost model,} selects the best performing \uprog \revdel{implementation of the desired operation} from the \uproglib. }

\gf{We compare the benefits of \prop to different state-of-the-art computing platforms (CPU, GPU, and the SIMDRAM~\cite{hajinazarsimdram} \gls{PuD} mechanism). 
We comprehensively evaluate \prop's
performance for \gfisca{twelve} real-world applications. 
Using a single DRAM bank, 
\gfisca{\prop provides 
\li~17$\times$, 7.3$\times$, and 10.2$\times$ the performance per mm$^2$; and
\lii~90.3$\times$, 21$\times$, and 8.1$\times$ \om{lower energy consumption than that} the CPU, GPU, and SIMDRAM, respectively, on average across all \om{twelve} real-world applications.}
\prop incurs low area cost on top of a DRAM chip (1.6\%) and CPU die (0.03\%).}
% \juan{As a result, \prop outperforms the state-of-the-art processing-using-DRAM approach.} 
% \kangqi{We demonstrate the superiority of \prop over CPU, GPU, and the state-of-the-art processing-using-DRAM approach, SIMDRAM, through micro-benchmarks like GEMV and real-world kernels like Neural Networks. Based on our evaluation, \prop outperforms the SIMDRAM baseline by (1) 1.5-12$\times$ and 1.2-6$\times$ for Vector Addition and Multiplication respectively; (2) 1-15$\times$ and 1-2$\times$ for reduction and GEMV kernel. In terms of Neural Networks, \prop is also capable of delivering maximally 2$\times$ performance and 8$\times$ power reduction over a high-end GPU. Nevertheless, \prop incurs a 2.5\% area overhead per DRAM bank}. 

\gf{We make the following key contributions:}
\begin{itemize}
[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,labelindent=0pt,itemindent=0pt,leftmargin=*]
\item \gf{To our knowledge, this is the first framework to enable \gls{PuD} operations with dynamic bit-precision, adaptive data representation, and flexible arithmetic.}

\item \gf{\prop provides a three-component framework to transparently 
\li~identify the bit-precision for a \gls{PuD} operation and 
\lii~select the best-performing implementation of the target \gls{PuD} operation based on the target bit-precision.} 

\item \gf{We extensively evaluate \prop \agy{for} twelve real-world applications\agy{, showing} that \prop %can 
outperforms state-of-the-art \gls{PuD} framework and processor-centric design while incurring low area \agy{cost} to the system.}
\end{itemize}

% As contemporary and emerging applications continue to generate massive amounts of data \cite{al2023big}, current computing paradigms struggle to handle it effectively. The energy and performance costs of moving data between the memory subsystem and the CPU constitute a significant proportion of the overall cost of computation \juan{\cite{mutlu2022modern, upmem2018, oliveira2021pimbench}}.
% % \jgl{When you have several citations in the same place, have them inside the same "cite"}. 
% % This situation necessitates radical revisions \jgl{No need to sound so "epic". See how I wrote the abstract.} to current computing methods. One approach that has gained increasing attention is the processing-in-memory (PIM) computing paradigm, which brings computation closer to the data, thereby reducing the costs of data movement.
% The processing-in-memory (PIM) paradigm has emerged as a promising solution to address the rising costs associated with data movement in modern computing systems. By strategically relocating computation closer to the data, PIM effectively minimizes the need for frequent data transfers between memory and processors, leading to enhanced cost efficiency. 
% % Modern memory systems provide new opportunities for architectures that can process data in the memory subsystem \cite{mutlu2014research}, but building PIM designs requires resolving practical system-level concerns, such as ensuring PIM is accessible to workloads and programmers. \jgl{Let's go to the point. Follow the same flow as the abstract.}

% One of the PIM architectures is Processing using DRAM 
% \jgl{Let's just use processing-using-DRAM consistently through the entire paper. No need to mention PnM or PuM in the intro (we can talk about them in the Related Work). See how the abstract flows from PIM to processing-using-DRAM. Intro should be the same.} \mayank{The point here is to mention that our framework is generalized and by changing the parameters we can find the new best approach for different kind of memory. But anyways I have changed it to DRAM. } 
% is a paradigm which leverages the inherent advantages of operating directly within memory arrays, capitalizing on their substantial internal bandwidth and parallelism. By performing computations in close proximity to the data, PIM harnesses the immense potential of memory arrays, resulting in significant performance benefits. This approach aims to minimize data movement and latency, improving overall system performance and energy efficiency. Processing-using-memory architectures uses bulk bitwise computation. This approach is particularly beneficial for data-intensive applications such as databases, neural networks, and graph analytics, which extensively utilize a diverse range of simple (e.g., AND, OR, XOR) and complex (e.g., equality check, multiplication, addition) bitwise operations. Ambit, an innovative in-DRAM processing-using-memory accelerator, introduced the groundbreaking concept of harnessing DRAM's analog operational principles to efficiently execute bulk bitwise AND, OR, and NOT logic operations. Through this pioneering work, Ambit paved the way for exploiting the inherent capabilities of DRAM and advancing the field of processing-using-memory architectures.
% \jgl{This paragraph should be about processing-using-DRAM approaches and what are their capabilities (e.g., type of operations they can do) and great promise.}\mayank{I have done some changes please check.}

% \jgl{This paragraph should talk about the limitations of existing processing-using-DRAM approaches. These are the three mentioned in the abstract. We need to elaborate a bit on each of them. About the data format, we can say that prior works are using 2's complement, which is normal on processor-centric systems, but do not consider that other formats may be more suitable for the processing-using-DRAM paradigm. About data precision, we have to say that prior works only consider powers-of-two, but this is not efficient for bit-serial algorithms, as we may operate on high-order bits that are not needed to represent small values. About the algorithms, we need to explain that only bit-serial computation has been used in most processing-using-DRAM approaches and those that use bit-parallel have very high area overheads (e.g., DRISA, DrAcc).} \mayank{I have done the edits, please check !!}In the majority of processing-using-DRAM approaches, the predominant method employed for computation is bit-serial computation. While this approach has been widely adopted, it is important to note that the utilization of bit-parallel computation is limited due to significant area overheads in existing solutions. For instance, approaches like DRISA and DrAcc, which incorporate bit-parallel computation, suffer from substantial area overheads that hinder their practical implementation. 

% Additionally, in general programming for Processing using DRAM (PIM) architectures, the data representation is typically done using static data formats. This means that the data is structured and stored in a fixed format, often predetermined by the architecture or system. Static data representation has its advantages, such as simplicity and efficient storage, as data can be organized and accessed in a predictable manner. However, it also has limitations in terms of flexibility and precision. One limitation is the fixed bit-precision of the data format which is not an efficient approach for bit-serial algorithms. In many applications, data processing operations may require a specific level of precision. However, with static data representation, the precision is predetermined and fixed. This can lead to inefficiencies when the required precision exceeds the available fixed format. For example, when performing an 8-bit accumulation, the fixed format may still require a 16-bit precision representation, leading to extra overhead in terms of memory and latency. Also for static data representation and fixed formats, the processing units often need to perform additional operations to handle the fixed format, resulting in increased latency. These additional operations can include data format conversions or precision adjustments, which can introduce overhead and impact overall computation time.

% Also, existing works in the field of processing-using-memory architectures commonly rely on the use of 2's complement representation, which is a conventional choice in processor-centric systems. However, these prior approaches often overlook the fact that alternative data formats may be more suitable for the processing-using-DRAM paradigm. This observation raises the need to explore and consider different data formats that can effectively leverage the unique characteristics and capabilities of DRAM-based processing.

% % Bit-serial processing is a technique that involves performing computations on data one bit at a time, sequentially, rather than processing the entire data word in parallel. In bit-serial processing, each bit of the data is processed individually, typically using shift registers or serial adders. When combining PuM and bit-serial processing, the idea is to perform bit-serial computations directly within the memory units themselves. This allows for highly parallel and distributed processing, as each memory unit can independently process a bit of the data in parallel with other memory units.

% % General programming for the PIM, whether it is a PuM (Processing using memory) or PnM (Processing near memory) is done via static data representation where data is structured and stored in a fixed format. But it lacks in terms of flexibility, fixed bit-precision which consume more bits (e.g. while performing 8-bit accumulation in some applications, we have use 16-bit precision format) and have high latency for computation. 

% % \jgl{Maybe you can reuse something in this paragraph to write what I explain in the previous paragraph.}


% % Also, current PuM architectures work in one subarray at a time without exploiting the parallelism that can be obtained from prior works like SALP, LISA, FIGARO etc. 

% % \jgl{The focus should not be on the prior works that we make use of. See my next comment.}
% % Also, in current Processing using Memory (PuM) architectures, the operation typically occurs in one subarray at a time, without fully exploiting the parallelism potential offered by prior works such as SALP (Scalable and Low-Power subarray level parallelism), LISA (Low-cost Interconnect subarray), FIGARO (Fine-Grained Reconfigurable Architecture). These prior works have proposed innovative approaches to enhance the parallelism and efficiency of PuM architectures. They introduce concepts such as SIMD (Single Instruction, Multiple Data) processing, reconfigurable architectures, and optimal computing to exploit parallelism and optimize performance.

% \jgl{After enumerating the limitations of existing processing-using-DRAM approaches, we have to introduce \prop{}. It is a flexible and adaptive framework that tackles the aforementioned limitations. Then, we need to describe the key ideas to deal with each of the limitations. Namely, (1) adaptive data format, (2) adaptive precision, (3) algorithm choice. Then, to make each key idea work, we need some key mechanisms. (1) For data format, we have a heuristic to select the best format and data format conversion mechanisms. (2) For adaptive precision, we can adapt the precision that an application needs at each point if we know what's the precision of the input. (3) For algorithm selection, we have performance models that indicate what's the best one based on the input size and we enable subarray-level parallelism (as proposed by SALP) and inter-subarray data movement (LISA, FIGARO) to support bit-parallel execution.} \mayank{I have written for it please take a look.}


% Therefore, we introduce \prop{}, an innovative framework that tackles limitations in processing-using-DRAM paradigms. It introduces adaptive data formats, adaptive precision, and algorithm choice to enhance flexibility and performance. The framework employs a heuristic-based approach and data format conversion mechanisms for adaptive data format selection which suits best for the application. Adaptive precision adjusts precision levels based on input precision, optimizing resource usage. Performance models guide algorithm selection, while subarray-level parallelism (as proposed by SALP) and inter-subarray data movement (as proposed by LISA) support efficient bit-parallel execution. \prop{} offers a comprehensive solution to overcome limitations, improving flexibility and efficiency in DRAM-based processing architectures.

% The evaluation results demonstrate the outstanding performance superiority of \prop{} compared to SIMDRAM, the state-of-the-art processing-using-DRAM approach, as well as traditional CPU and GPU architectures. Through extensive micro benchmarks, such as GEMV, and real-world kernel applications like Neural Networks, \prop{} consistently outperforms SIMDRAM. For Vector Addition and Multiplication, \prop{} achieves remarkable improvements of 1.5-12$\times$ and 1.2-6$\times$, respectively. Moreover, for reduction and GEMV kernel operations, \prop{} delivers significant enhancements of 1-15$\times$ and 1-2$\times$, respectively. Additionally, \prop{} showcases exceptional performance by outperforming a high-end GPU implementation of the efficient Neural Network, MobileNets, with a 2$\times$ performance boost and 8× superior power consumption. Despite incurring a modest 2.5\% area overhead only over the conventional DRAM architecture and <0.2 $\%$ over a high-end CPU, \prop{} proves to be an impressive and promising solution for processing-using-DRAM architectures, surpassing the state-of-the-art with its remarkable performance gains. To achieve diverse tradeoffs between high throughput, high latency, and low energy consumption, we 
% implemented a variety of complex parallel algorithms, adaptive precision approaches, and different data format representations to leverage parallelism and introduce flexibility in current DRAM technologies. We designed our framework on performance models of different algorithms, and representations and introduced optimizations such as adaptive data precision with support for different types of DRAM substrate (e.g. DDR-3, DDR-4, HBM etc.) \jgl{Do we really have different DRAM technologies?} \mayank{Yes, we do create different parameters for different technologies and based on that results can change}. 
% % \gfb{Present the problem concretely first. From the previous paragraph, I didn't know that data layout was a problem. A compiler itself does not solve all system-level concerns one can imagine. Only a particular one. Be clear about that particular one.}
% % \gfb{
% % 1. Introduce PUM.
% % 2. Explain that PUM does bit-serial computation over transposed data.
% % 3. Other PUM architectures have been proposed for data movement acceleration.
% % 4. Explain the limitations of 2, which should lead to the problem statement.}
% % \jgl{We do not need this paragraph. We need a summary of results (the same as in abstract or a bit more detail).}
% % Therefore, we aim to address these practical system-level concerns by developing a compiler \mayank{Again what should we call here} \prop{} that can efficiently map data into different layouts for processing and can also provide dynamic precision for widely intensive data application (e.g. Neural networks, Databases etc.). Previous research has shown that laying out data vertically can enhance system throughput \cite{}. However, the SIMDRAM \cite{hajinazarsimdram} paper introduced the concept of processing data vertically and implemented various complex operations without fully utilizing parallelism available in other works such as LISA \cite{chang2016low}, SALP \cite{salp} and FIGARO \cite{wang2020figaro}. 
% % To achieve diverse tradeoffs between high throughput, high latency, and low energy consumption, we 
% % % \gfb{Don't use future tense. Always present tense, active voice.} 
% % implemented a variety of complex algorithms that leverage parallelism in current memory technologies.

% % \gfb{Missing key idea, key insight, clear key mechanism and key results.}
% % We also explored different data representation techniques such as 2's complement \cite{baugh1973two} and Redundant Binary representation (RBR) and different types of computational algorithms for addition and multiplication that can be utilized to perform different complex operations. On top of it, we analyzed these different representation with variety of bitserial and bitparallel algorithms that adhere to different data layout and evaluate them on Micro-benchmarks like Vector operations, GemV and also for real workloads like neural networks. We designed our compiler to support different types of DRAM substrate (e.g. DDR-3, DDR-4, HBM etc.) \jgl{Do we really have different DRAM technologies?}. We evaluate the overall area overhead in the evaluation section and observe that our substrate has <2.5 $\%$ area overhead only over the conventional DRAM architecture and <0.2 $\%$ over a high-end CPU. This includes the \prop{} compiler hardware infrastructure. \mayank{Add few results here.}

% We make the following contributions. \jgl{We'll need better writing here.} \mayank{I have edited it please check !!}
% % \begin{itemize}
% %     \item We propose a new framework \jgl{Let's just call it framework. We do not really have a compiler.} framework \prop{} which can efficiently map the given data-intensive application according to the user preference for different tradeoffs among latency, energy and throughput. 
% %     \item We showcase implementation of various bit-serial and bit parallel algorithms for addition and multiplication (but can be extended to perform any kind of complex algorithms) for different data representations techniques.
% %     \item We also performed and present the data parallelism and optimization using our \prop{} substrate which can enable extensive parallelism and optimization in mapping of data for many real-world data intensive applications.
% %     \item Also, we propose a dynamic bit-precision technique on our \prop{} substrate using our compiler efficiently perform the data bit-width changing operations like Accumulation and showcase the improvement upon static data representation. 
% % \end{itemize}
% \begin{itemize}
% \item Framework: We propose a novel framework called \prop{}, designed to efficiently map data-intensive applications while considering user preferences for latency, energy consumption, and throughput tradeoffs. This framework provides flexibility in optimizing the mapping of applications, enabling customization according to specific requirements.

% \item Algorithm Implementation: We demonstrate the implementation of various bit-serial and bit-parallel algorithms for addition and multiplication, which can be extended to handle complex algorithms. These algorithms utilize different data representation techniques, showcasing the versatility of \prop{} in accommodating diverse data processing requirements.

% \item Data Parallelism and Optimization: Our \prop{} substrate enables extensive data parallelism and optimization for mapping data in a wide range of real-world data-intensive applications. Leveraging the capabilities of \prop{}, we achieve significant improvements in both parallelism and optimization, enhancing overall application performance.

% \item 
% Dynamic Bit-Precision Technique: To further enhance data representation, we propose a dynamic bit-precision technique using our \prop{} compiler. This technique efficiently performs data bit-width changing operations, such as accumulation, enabling adaptive precision based on specific application. Through this dynamic approach, we demonstrate improvements over static data representation techniques, showcasing the benefits of utilizing \prop{} in data-intensive computations.

% \end{itemize}

% By presenting this comprehensive framework and its associated techniques, we provide a flexible and adaptive solution for efficiently mapping data-intensive applications while considering latency, energy, and throughput tradeoffs. Overall, this research aims to contribute to the development of efficient PIM designs that can handle the ever-growing amounts of data generated by contemporary and emerging applications.

% % \cite{kuninobu1987design}. Additionally, we will analyze various adder types, including Ripple carry adder \cite{chang1998carry}, Sklansky adder \cite{sankar2013design}, Kogge stone adder \cite{chakali2013design}, Brent Kung adder \cite{saxena2015design}, Ladner Fischer adder \cite{fariddin2013design}, Carry Select adder \cite{bedrij1962carry}, and Redundant binary adder \cite{chow1978logical}. Moreover, we will investigate different multiplication algorithms such as Shift and add multiplication \cite{gwee2008low} and karatsuba multiplication \cite{fang2007karatsuba}. 
% % We will also examine different versions of these multipliers that incorporate various types of adders.

 
 

% % \gfb{Contribution list:}

==> mainmatter/06_proteus/sections/06_related.tex <==
\section{Related Work}

To our knowledge, \prop is the first work that provides the hardware support to transparently execute \gls{PuD} operations with the most bit-precision and arithmetic.  We highlight \prop's key contributions by contrasting them with state-of-the-art \gls{PIM} designs. 


\paratitle{Processing-Using-DRAM} 
\gf{Prior works propose different ways of implementing \gls{PuD} operations~\cite{seshadri2013rowclone,seshadri2017ambit,xin2020elp2im,deng2018dracc,gao2019computedram,angizi2019graphide,hajinazarsimdram,li2018scope,ferreira2022pluto,deng2019lacc,kim2019d,li2017drisa,zhou2022flexidram, mimdramextended}\revdel{, either by 
\li~using the memory arrays themselves to perform  operations in bulk~\cite{seshadri.bookchapter17, seshadri2013rowclone,seshadri2018rowclone,chang2016low,wang2020figaro,seshadri2017ambit, xin2020elp2im, besta2021sisa,deng2018dracc, gao2019computedram,li2017drisa,angizi2019graphide, hajinazarsimdram,li2018scope,ferreira2021pluto,ferreira2022pluto,deng2019lacc,olgun2021quactrng,bostanci2022dr,kim2019d};
\lii~modifying the DRAM sense amplifier design with logic gates for computation~\cite{li2017drisa,zhou2022flexidram}}. 
\revdel{Even though such works leverage different algorithms and execution models to implement \gls{PuD} operations, they all assume a fixed bit-precision and algorithmic implementation. To improve performance,} Such works could benefit from \prop's dynamic bit-precision selection and alternative data representation and algorithms, since they all assume a static bit-precision and algorithmic implementation.
\gfisca{AritPIM~\cite{leitersdorf2023aritpim} provides a collection of bit-parallel and bit-serial algorithms for \gls{PuM} arithmetic. Compared to AritPIM, \prop
\li~implements a collection of other bit-parallel algorithms for \gls{PuM};
\lii~evaluates different data format representations that can lead to further performance and energy improvements; 
\liii~proposes a framework that can dynamically adapt to the bit-precision of the operation.}} 

\paratitle{Using Bit-Slicing Compilers \asplosrev{\hl{\& Early Termination}} for \gls{PIM}} \gf{Prior works~\cite{peng2023chopper,arora2023comefa} propose bit-slicing compilers for bit-serial \gls{PIM} computation. In particular, CHOPPER~\cite{peng2023chopper} improves SIMDRAM's programming model by leveraging bit-slicing compilers and employing optimizations to reduce the latency of a \uprog\revdel{, such as employing \gls{BLP} to overlap the latency of data copy and computation for \gls{PuD} operations targeting different DRAM banks}. Compared to CHOPPER, \prop has two main advantages. 
First, \prop improves a \uprog performance by \emph{fully} leveraging the DRAM parallelism within a single DRAM bank.\revdel{ In fact, the method CHOPPER proposes to exploit \gls{BLP} is already enabled by most memory controllers (i.e., a memory controller already parallelizes DRAM requests targeting different DRAM banks).} 
Second, although bit-slicing compilers can naturally adapt to different bit-precision values, they require the programmer to specify the target bit-precision manually. In contrast, \prop dynamically identifies the most suitable bit-precision transparently from the programmer.}
\asplosrev{\hl{Some other prior works (e.g.,~\mbox{\cite{caminal2022accelerating, wong2023pumice}}) propose techniques to realize early termination of \mbox{\gls{PuM}} operations for different memory technologies. Compared to these, \mbox{\prop}'s main novelty lies in realizing early termination of bit-serial operation in the context of DRAM/majority-based \mbox{\gls{PuD}} systems.}}


% \paratitle{Using Bit-Slicing Compilers for \gls{PIM}} 
%  Prior works propose different programming models for different types of \gls{PuM} architectures, as for example
% \li~CUDA/OpenAcc~\cite{cheng2014professional, OpenACCA1:online} for in-cache computing~\cite{dualitycache};
% \lii~tensor dataflow graphs for in-cache~\cite{wang2023infinity} and in-ReRAM computing~\cite{fujiki2018memory}. By enabling fine-grained DRAM, we believe such programming models can be ported to \gfi{\gls{PuD}} computing (for example, by assuming that each DRAM mat executes a different CUDA thread block). 

==> mainmatter/07_dappa/packages_dappa.tex <==

\usepackage[normalem]{ulem}
%\usepackage{multirow}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%\usepackage{stmaryrd}
%\usepackage{amsmath}
%\usepackage{listings}
\usepackage{subcaption}
\usepackage{clipboard}
\usepackage{soul}
%\usepackage[super]{nth}
\usepackage{tikz}
\usepackage{flushend}
%\usepackage[table,xcdraw]{xcolor}
%\usepackage[noadjust]{cite}
\usepackage{xargs} 
%\usepackage{todonotes}
%\usepackage[binary-units=true]{siunitx}
%\usepackage{tikzducks}
%\usepackage{duckuments}
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage{booktabs}
\usepackage{multirow}
%\usepackage{siunitx}
\usepackage[many]{tcolorbox}% version 2.80 (2014/03/31)
\usepackage{longfbox}

\usepackage{listings}
\definecolor{LightGray}{gray}{0.95}


%\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{pifont}
\usepackage[acronym,nonumberlist,nowarn]{glossaries}
    \glsdisablehyper
     \loadglsentries{support/acronyms}


\usepackage{xspace}
\usepackage[binary-units=true]{siunitx}
\usepackage{todonotes}

\usepackage{balance}


%\newcommand{\subparagraph}{}

%\usepackage[explicit]{titlesec}
\usepackage{setspace}
\usepackage[export]{adjustbox}

\usepackage{fancyhdr}
%\usepackage[hyphens]{url}


\usepackage{cleveref}
\crefformat{section}{\S#2#1#3}
\crefformat{subsection}{\S#2#1#3}
\crefformat{subsubsection}{\S#2#1#3}

%\usepackage{hyperref}

%\hypersetup{
%  colorlinks   = true, %Colours links instead of ugly boxes
%  urlcolor     = blue, %Colour for external hyperlinks
%  linkcolor    = blue, %Colour of internal links
%  citecolor   = black %Colour of citations
% }



==> mainmatter/07_dappa/sections/00_abstract.tex <==
\begin{abstract}


The growing volume of data in modern applications has led to significant computational costs in conventional processor-centric systems. 
Processing-in-memory (PIM) architectures alleviate these costs by moving computation closer to memory, reducing data movement overheads. UPMEM is the first commercially available PIM system, featuring thousands of in-order processors (DPUs) integrated within DRAM modules. However, programming a UPMEM-based system remains challenging due to the need for explicit data management and workload partitioning across DPUs.

We introduce \prop (\underline{da}ta-\underline{p}arallel~\underline{p}rocessing-in-memory \underline{a}rchitecture), a programming framework that eases the programmability of UPMEM systems by automatically managing data movement, memory allocation, and workload distribution. 
The \emph{key idea} behind \prop is to leverage a high-level data-parallel pattern-based programming interface to abstract hardware complexities away from the programmer. 
\prop comprises three main components:
\li~\emph{data-parallel pattern APIs}, a collection of five primary data-parallel pattern primitives that allows the programmer to express data transformations within an application;
\lii~a \emph{dataflow programming interface}, which allows the programmer to define how data moves across data-parallel patterns; and
\liii~a \emph{dynamic template-based compilation}, which leverages code skeletons and dynamic code transformations to convert data-parallel patterns implemented via the dataflow programming interface into an optimized UPMEM binary. 
%\prop supports five key data-parallel patterns—\texttt{map}, \texttt{filter}, \texttt{reduce}, \texttt{window}, and \texttt{group}—allowing users to describe complex computations without explicit hardware knowledge.

We evaluate \prop using six workloads from the PrIM benchmark suite on a real UPMEM system. Compared to hand-tuned implementations, \prop improves end-to-end performance by 2.1$\times$, on average, and reduces programming complexity (measured in lines-of-code) by 94\%. Our results demonstrate that \prop is an effective programming framework for efficient and user-friendly programming on UPMEM systems.

\end{abstract}

==> mainmatter/07_dappa/sections/01_introduction.tex <==
\glsresetall

\section{Introduction}
\label{sec:introduction}

The increasing prevalence and growing size of data in modern applications have led to high costs for computation in traditional \emph{processor-centric computing} systems~\cite{mutlu2013memory,
mutlu2015research,
dean2013tail,
kanev_isca2015,
mutlu2019enabling,
mutlu2019processing,
mutlu2020intelligent,
ghose.ibmjrd19,
mutlu2020modern,
boroumand2018google, 
wang2016reducing, 
mckee2004reflections,
wilkes2001memory,
kim2012case,
wulf1995hitting,
ghose.sigmetrics20,
ahn2015scalable,
PEI,
sites1996,
deoliveira2021IEEE}. 
To mitigate these costs, the \emph{processing-in-memory} (PIM)~\pimdef paradigm moves computation closer to where the  data resides, reducing the need to move data between memory and the processor. 
Even though the concept of PIM has been first proposed in the 1960s~\cite{Kautz1969,stone1970logic}, and various PIM architectures have been proposed since then~\pimall, real-world PIM systems have only recently been manufactured~\cite{upmem,upmem2018,kwon202125, lee2021hardware,ke2021near}; from which the UPMEM PIM system~\cite{upmem,upmem2018,gomez2021benchmarking} is the first PIM architecture to become commercially available. 
It consists of \emph{UPMEM modules}, which are standard DDR4-2400 DIMMs with 16 PIM chips. A \emph{PIM chip} consists of eight small multithreaded general-purpose in-order processors called DPUs. 
Each \emph{DPU} has exclusive access to 
a \SI{64}{\mega\byte} DRAM bank (called \emph{MRAM}), 
a \SI{24}{\kilo\byte} instruction memory (called \emph{IRAM}), and a \SI{64}{\kilo\byte} scratchpad memory (called \emph{WRAM}).
A common UPEM-capable system has 20 DRAM modules with 128 DPUs and \SI{8}{\giga\byte} of memory each, totaling 2,560 DPUs with \SI{160}{\giga\byte} of memory.

To program the DPUs in a UPMEM-capable system, UPMEM has developed a single-instruction multiple-thread (SIMT) programming model. 
The programming model uses a C-like interface and exposes to the programmer a series of application programming interfaces (APIs) to manage data allocation and data movement between the host CPU/DPUs and within the memory hierarchy of the DPUs. 
A programmer needs to follow four main steps to implement a given application targeting the UPMEM system. The programmer needs to: 
\li~partition the computation (and input data) across the DPUs in the system, \emph{manually} exposing thread-level parallelism (TLP);
\lii~distribute (copy) the appropriate input data from the CPU's main memory into the DPU's memory space;
\liii~launch the computation kernel that the DPUs will execute; and
\liv~gather (copy) output data from the DPUs to the CPU main memory once the DPUs execute the kernel.

Even though UPMEM's programming model resembles that of widely employed architectures, such as GPUs, it requires the programmer to 
\li~have prior knowledge of the underlying UPMEM hardware and
\lii~manage data movement at a fine-grained granularity \emph{manually}. 
Such limitations can difficult the adoption of PIM architectures in general-purpose systems. 
Therefore, our \textbf{goal} in this work is to ease programmability for the UPMEM architecture, allowing a programmer to write efficient PIM-friendly code \emph{without} the need to manage hardware resources explicitly. 

To ease the programmability of PIM architectures, we propose \prop (\underline{da}ta-\underline{p}arallel \underline{p}rocessing-in-memory \underline{a}rchitecture), a programming framework that can, for a given application, \emph{automatically} distribute input and gather output data, handle memory management, and parallelize work across the DPUs. 
The \emph{key idea} behind \prop is to remove the responsibility of managing hardware resources from the programmer by providing an intuitive data-parallel pattern-based programming interface~\cite{cole1989algorithmic,cole2004bringing}, which abstracts the hardware components of the UPMEM system. 
Using this key idea, \prop transforms a data-parallel pattern-based application code into the appropriate UPMEM-target code, including the required APIs for data management and code partition, which can then be compiled into a UPMEM-based binary \emph{transparently} from the programmer. 
While generating UPMEM-target code, \prop implements several code optimizations to improve performance.

Concretely, \prop takes as input C/C++ code, which describes the target computation using a collection of data-parallel patterns and \prop's programming interface, and generates as output the requested computation. \prop consists of three main components:
\li~\prop's data-parallel pattern APIs,
\lii~\prop's dataflow programming interface, and
\liii~\prop's dynamic template-based compilation.
\prop's \textbf{data-parallel pattern APIs} are a collection of pre-defined functions that implement high-level data-parallel pattern primitives~\cite{cole1989algorithmic,cole2004bringing}. 
Each primitive allows the user to express how data is transformed during computation. \prop supports five primary data-parallel pattern primitives, including \texttt{map}, \texttt{filter}, \texttt{reduce}, \texttt{window}, and \texttt{group}.  
The user can combine data-parallel primitives to describe complex data transformations in an application. \prop is responsible for translating and parallelizing each data-parallel primitive to efficient CPU and UPMEM code. 
\prop exposes a \textbf{dataflow programming interface} to the user. 
In this programming interface, the main component is the \texttt{Pipeline} class, which represents a sequence of data-parallel patterns that will be executed on the DPUs. A given \texttt{Pipeline} has one or more \texttt{stage}s. Each \texttt{stage} utilizes a given data-parallel pattern primitive to transform input operands following a user-defined computation. \texttt{Stage}s are executed in order, in a pipeline fashion. 
Finally, \prop uses a \textbf{dynamic template-based compilation} to generate UPMEM code in two main steps.
In the first step, \prop creates an initial UPMEM code based on code skeletons of a UPMEM application. 
In the second step, \prop uses a series of transformations to 
\li~extract the required information that will be fed to the UPMEM code skeletons from the user program; 
\lii~calculate the appropriate offsets used when managing data across MRAMs and WRAMs; and
\liii~divide computation between CPU and DPUs. 
Using \prop's data-parallel pattern APIs, dataflow programming interface, and dynamic template-based compilation, the user can quickly implement and deploy applications to the UPMEM system without any knowledge of the underlying architecture. 

To demonstrate \prop's benefits, we implement a subset of the workloads (i.e., vector addition, select, reduction, unique, imagine histogram small, and general matrix-vector multiplication) presented in the UPMEM-based PrIM benchmark suite~\cite{gomezluna2021repo} using our data-parallel pattern model. 
We perform our evaluation on a UPMEM PIM system that includes a 2-socket Intel Xeon Silver 4110 CPU at \SI{2.10}{\giga\hertz} (host CPU), standard main memory (DDR4-2400) of \SI{128}{\giga\byte}, and 20 UPMEM PIM DIMMs with \SI{160}{\giga\byte} PIM-capable memory and 2,560 DPUs. We compare \prop's performance and programming complexity to that of the hand-tuned implementations present in PrIM.
First, compared to hand-tuned PrIM workloads, \prop improves end-to-end performance by 2.1$\times$, on average across the six workloads. \prop's performance improvement is due to code optimizations, such as parallel data transfer and partitioning of workload between CPU and DPU. 
Second, \prop \emph{significantly} reduces programming complexity (measured by lines-of-code) on average by 94\%. We conclude that \prop is an efficient programming framework that eases the programmability of the UPMEM PIM architecture. 


We make the following key contributions:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,labelindent=0pt,itemindent=0pt,leftmargin=*] 
    \item To our knowledge, this is the first work to propose a data-parallel pattern-based programming framework that abstracts \emph{both} computation and communication requirements while  \emph{automatically} generating code for the UPMEM architecture. \

    \item We propose \prop (\underline{da}ta-\underline{p}arallel~\underline{p}rocessing-in-memory \underline{a}rchitecture), a programming framework that \emph{automatically} distributes input and gathers output data, handles memory management, and parallelizes work across DPUs.

    \item We equip \prop with a series of code optimizations that improve the performance of workloads running on the UPMEM system.

    \item We evaluate \prop using six workloads from the PrIM benchmark suite, and we observe that \prop improves performance by 2.1$\times$ and reduces lines-of-code by 94\%, on average, compared to the hand-tuned PrIM workloads.
\end{itemize}

==> mainmatter/07_dappa/sections/06_related.tex <==
\section{Related Work}

To our knowledge, \prop is the first data-parallel pattern-based programming framework to generate code for the UPMEM architecture \emph{fully} automatically.
We first review works that provide high-level programming frameworks or APIs for the UPMEM system. Second, we discuss compiler solutions targeting PIM architectures.

\paratitle{Programming Frameworks/APIs for UPMEM} Several prior works~\cite{chen2023simplepim,item2023transpimlib,giannoula2024pygim} propose different programming frameworks or APIs to ease programmability in UPMEM-based PIM systems. 
First, SimplePIM~\cite{chen2023simplepim} proposes a high-level programming framework that encapsulate management, computation, and communication primitives into software APIs. Similarly to \prop, SimplePIM uses a MapReduce-like programming model~\cite{jiang2010map}, with support for three execution parallel patterns (i.e., \texttt{map}, \texttt{reduce}, and \texttt{zip}). 
\prop builds on top of SimplePIM by 
\li~further extending the programming model to allow for native implementation of more parallel patterns,
\lii~\emph{completely} eliminating the need for the user to handle data communication between CPU and DPUs and across DPUs, and
\liii~allowing for \emph{automatic} cooperative execution between CPU and DPUs for a given kernel. 
By doing so, \prop further improves programming productivity compared to SimplePIM (as we show in Section~\ref{sec:eval}).
Second, other works, such as TransPimLib~\cite{item2023transpimlib} and PyGim~\cite{giannoula2024pygim}, provide implementation support for key computation kernels, such as transcendental functions and graph neural networks. 
Even though such works also aid UPMEM programmability, they are limited to a narrow application scope. 

\paratitle{Compiler Support for PIM} Many prior works propose compiler solutions for different PIM systems~\cite{hadidi2017cairo,mimdramextended,ahmed2019compiler,peng2023chopper,wang2023infinity,dualitycache,zha2020hyper,fujiki2018memory}. However, none of such compilers is suitable for the real UPMEM PIM system. 
The authors of~\cite{khan2022cinm} propose CINM, a compiler based on MLIR~\cite{lattner2021mlir} (multi-level intermediate representation) for both UPMEM-like PIM systems and analog-based PIM architectures. Compared to \prop, its main limitation is the fact that it only supports linear algebra PIM kernels.

==> mainmatter/zusammenfassung.tex <==
\vspace{-3em}\chapter*{Zusammenfassung}
\addcontentsline{toc}{chapter}{Zusammenfassung}

The increasing prevalence and growing size of data in modern applications have led to high performance and energy costs for computation in traditional processor-centric computing systems. To mitigate these costs, the processing-in-memory (PIM) paradigm moves computation closer to where the data resides, reducing (and sometimes eliminating) the need to move data between memory and the processor. There are two main approaches to PIM: (1) processing-near-memory (PNM), where PIM logic is added to the same die as memory or to the logic layer of 3D-stacked memory, and (2) processing-using-memory (PUM), which uses the operational principles of memory cells and memory circuitry to perform computation.
Many works from academia and industry have shown the benefits of PNM and PUM for a wide range of workloads from different domains. However, fully adopting PIM in commercial systems is still very challenging due to the lack of tools and system support for PIM architectures across the computer architecture stack, which includes: (i) workload characterization methodologies and benchmark suites targeting PIM architectures; (ii) execution models that can take advantage of the available application parallelism to maximize hardware utilization and throughput; (iii) compiler support and compiler optimizations targeting PUM architectures;  (iv) data-aware runtime systems that can leverage key characteristics of PIM-friendly data to improve overall performance and energy efficiency. 

Unser Ziel in dieser Dissertation ist es, Werkzeuge und Systemunterstützung für PIM-Architekturen (mit Schwerpunkt auf DRAM-basierten Lösungen) bereitzustellen, um die Einführung solcher Architekturen in aktuellen und zukünftigen Systemen zu erleichtern.  
Zu diesem Zweck stellen wir zunächst DAMOV vor, die erste rigorose Methode zur Charakterisierung von Engpässen bei speicherbezogenen Datenbewegungen in modernen Workloads, sowie die erste Benchmark-Suite für Datenbewegungen.
In DAMOV führen wir (i) die erste groß angelegte Charakterisierung von Anwendungen durch, um eine dreistufige Workload-Charakterisierungsmethode zu entwickeln, die vier Schlüsselmetriken einführt und auswertet, um die Quellen von Datenbewegungsengpässen in realen Anwendungen zu identifizieren, und (ii) untersuchen, ob PIM-Architekturen ein praktikabler Mechanismus zur Abschwächung von Datenbewegungen für verschiedene Klassen von Anwendungen mit Speicherengpässen sind.
Zweitens gehen wir mit MIMDRAM auf die derzeitigen Beschränkungen des massiven bitweisen Ausführungsmodells von PUD-Architekturen (Processing-Using-DRAM) ein. MIMDRAM ist ein von Hardware und Software gemeinsam entwickeltes PUD-Substrat, das nur die benötigten Rechenressourcen im DRAM für PUD-Rechenaufgaben zuweisen und steuern kann. Auf der Hardwareseite führt MIMDRAM einfache Änderungen an der DRAM-Architektur ein, die die gleichzeitige Ausführung (i) verschiedener PUD-Operationen in einem einzigen DRAM-Subarray in einer Multiple-Instruction-Multiple-Data
(MIMD) und (ii) native Vektorreduktionsberechnungen ermöglichen.
Softwareseitig implementiert MIMDRAM eine Reihe von Compilerdurchläufen, die automatisch Codebereiche identifizieren und auf das zugrunde liegende PUD-Substrat abbilden, sowie Systemunterstützung für die Datenabbildung und Zuweisung von PUD-Speicherobjekten.
Drittens adressieren wir in Proteus die hohe Latenz, die durch die Ausführung von massiven bitweisen PUD-Operationen in modernen PUD-Architekturen entsteht, indem wir eine datenbewusste Laufzeit-Engine für PUD implementieren. Konkret reduziert Proteus die Latenz von PUD-Operationen durch (i) Parallelisierung der Ausführung von datenunabhängigen Primitiven in einer PUD-Operation und (ii) Reduzierung der Bitgenauigkeit für PUD-Operationen unter Ausnutzung von schmalen Werten (d.h. Werte mit vielen führenden Nullen oder Einsen).
Viertens erleichtern wir mit DaPPA die Programmierbarkeit einer kommerziellen Allzweck-PNM-Architektur, indem wir dem Programmierer die Möglichkeit geben, effizienten PIM-freundlichen Code zu schreiben, ohne dass er Hardware-Ressourcen explizit verwalten muss. Die Schlüsselidee hinter DaPPA ist es, dem Programmierer die Verantwortung für die Verwaltung von Hardwareressourcen abzunehmen, indem wir
eine intuitive, auf datenparallelen Mustern basierende Programmierschnittstelle, die die Hardwarekomponenten des PNM-Systems abstrahiert. Mit dieser Schlüsselidee verwandelt DaPPA einen
DaPPA wandelt einen auf datenparallelen Mustern basierenden Anwendungscode in den entsprechenden PNM-Zielcode um, einschließlich der erforderlichen APIs für die Datenverwaltung und Codepartitionierung, der dann vom Programmierer transparent in eine PNM-basierte Binärdatei kompiliert werden kann.

==> support/placeholder_macros.tex <==
\newcommand{\nind}[0]{\noindent}
\newcommand{\head}[1]{\noindent\textbf{#1.}}
\newcommand{\qhead}[1]{\noindent\textbf{#1?}}


==> support/sorted_citationblocks.tex <==
\newcommand{\rhmemisolationrefs}[0]{\cite{aga2017when, agarwal2018rowhammer_for, barenghi2018softwareonly, bhattacharya2016curious, bhattacharya2018advanced, bosman2016dedup, brasser2017cant, burleson2016invited, carre2018openssl, cohen2022hammerscope, cojocar2019exploiting, cojocar2020arewe, deridder2021smash, fahrjr2022when, fournaris2017exploiting, frigo2018grand, frigo2020trrespass, genssler2022onthe, gruss2015rowhammerjs_a, gruss2018another, hassan2021uncovering, hong2019terminal, jang2017sgxbomb, jattke2022blacksmith, ji2019pinpoint, khan2018analysis, kim2014flipping, kim2020revisiting, kogler2022halfdouble, kwong2020rambleed, li2014write, lim2017active, lipp2018nethammer, liu2022generating, mutlu2017therowhammer, mutlu2019rowhammer_a, mutlu2023fundamentally, ni2018write, orosa2021adeeper, orosa2022spyhammer, park2016experiments, park2016statistical, pessl2016drama_exploiting, poddebniak2018attacking, qiao2016anew, rakin2022deepsteal, razavi2016flip, ryu2017overcoming, safari2014rowhammer, seaborn2015exploiting, tatar2018defeating, tatar2018throwhammer, tobah2022spechammer, tol2022toward, vanderveen2016drammer_deterministic, vanderveen2018guardion, walker2021ondram, weissman2020jackhammer, xiao2016onebit, yaglikci2022understanding, yang2019trapassisted, yao2020deephammer, yun2018study, zhang2018triggering, zhang2020pthammer, zhang2022implicit, zheng2023trojvit}}

\newcommand{\exploitingRowHammerAllCitations}[0]{\cite{aga2017when, aydin2022cyber, barenghi2018softwareonly, bhattacharya2016curious, bhattacharya2018advanced, bosman2016dedup, brasser2017cant, burleson2016invited, cai2022onthe, carre2018openssl, cohen2022hammerscope, cojocar2019exploiting, cojocar2020arewe, deridder2021smash, fahr2022theeffects, fahrjr2022when, fournaris2017exploiting, france2022modeling, frigo2018grand, frigo2020trrespass, gruss2015rowhammerjs_a, gruss2018another, hassan2021uncovering, hong2019terminal, islam2022signature, jang2017sgxbomb, jattke2022blacksmith, ji2019pinpoint, kaur2022workinprogress, kim2014flipping, kogler2022halfdouble, kwong2020rambleed, lefforge2023reverse, li2022cyberradar, li2023fphammer, lipp2018nethammer, liu2022generating, mus2022jolt, mutlu2017therowhammer, mutlu2019rowhammer_a, orosa2022spyhammer, pessl2016drama_exploiting, poddebniak2018attacking, qiao2016anew, rakin2022deepsteal, razavi2016flip, roohi2022efficient, safari2014rowhammer, seaborn2015exploiting, staudigl2022neurohammer, tatar2018defeating, tatar2018throwhammer, tobah2022spechammer, tol2022toward, tomita2022extracting, vanderveen2016drammer_deterministic, vanderveen2018guardion, wang2022research, weissman2020jackhammer, xiao2016onebit, yang2022sociallyaware, yao2020deephammer, zhang2018triggering, zhang2020pthammer, zhang2022implicit, zheng2023trojvit}}

\newcommand{\trrCitations}[0]{\cite{bennett2021panopticon, devaux2021method, jedec2020jesd2095a, jedec2020jesd794c, lee2014green, micron2016ddr4, yaglikci2021security}}

\newcommand{\understandingRowHammerAllCitations}[0]{\cite{agarwal2018rowhammer_for, baeg2022estimation, cohen2022hammerscope, frigo2020trrespass, gautam2019rowhammering, genssler2022onthe, he2023whistleblower, jiang2021quantifying, khan2018analysis, kim2014flipping, kim2020revisiting, li2014write, lim2017active, lim2018study, luo2023rowpress, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_a, mutlu2023fundamentally, ni2018write, olgun2023anexperimental, olgun2023dram_bender, orosa2022spyhammer, park2014activeprecharge, park2016experiments, park2016statistical, redeker2002aninvestigation, ryu2017overcoming, walker2021ondram, yang2016suppression, yang2017scanning, yang2019trapassisted, yun2018study, zhou2023doublesided, zhou2024unveiling, zhou2024understanding, li2023understanding}}

\newcommand{\understandingRowHammerNVMCitations}[0]{\cite{agarwal2018rowhammer_for, genssler2022onthe, khan2018analysis, li2014write, ni2018write}}

\newcommand{\understandingRowHammerSimulationCitataions}[0]{\cite{gautam2019rowhammering, jiang2021quantifying, redeker2002aninvestigation, ryu2017overcoming, walker2021ondram, yang2016suppression, yang2017scanning, yang2019trapassisted}}

\newcommand{\mitigatingRowHammerAllCitations}[0]{\cite{aichinger2015ddrmemory, ajorpaz2022evax, apple2015about, arikan2022processor, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, bennett2021panopticon, bostanci2024comet, brasser2017cant, devaux2021method, didio2023copyonflip, enomoto2022efficient, enterprise2015hpmoonshot, fakhrzadehgan2022safeguard, france2022modeling, france2022reducing, frigo2020trrespass, gautam2019rowhammering, gomez2016dram_rowhammer, greenfield2012throttling, guderamarao2023defending, guha2022criticality, han2021surround, hassan2019crow, hassan2021uncovering, hassan2024acase, hong2023dsac, irazoqui2016mascat, jedec2020jesd794c, jedec2020jesd795, joardar2022learning, joardar2022machine, juffinger2023csirowhammercryptographic, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, kim2023a11v, konoth2018zebram, lee2019twice, lee2021cryoguard, lenovo2015rowhammer, loughlin2021stop, loughlin2022moesiprime, manzhosov2022revisiting, marazzi2022rega, marazzi2023protrr, mutlu2023fundamentally, naseredini2022alarm, olgun2024abacus, park2020graphene, park2022rowhammer_reduction, qureshi2022hydra, ryu2017overcoming, saileshwar2022randomized, saroiu2022howto, saroiu2022theprice, saxena2022aqua, saxena2023ptguard, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, sharma2022areview, son2017making, tomita2022extracting, vanderveen2018guardion, vig2018rapid, wi2023shadow, woo2023scalable, yaglikci2021blockhammer, yaglikci2021security, yaglikci2022hira, yang2016suppression, yang2017scanning, you2019mrloc, zhang2020leveraging, zhang2022softtrr, zhou2022ltpim, zhou2023dnndefender}}

\newcommand{\hwBasedRowHammerMitigations}[0]{\cite{aichinger2015ddrmemory, ajorpaz2022evax, apple2015about, arikan2022processor, aweke2016anvil, bains2015method, bains2015rowhammer, bains2016distributed, bains2016rowhammer, bennett2021panopticon, bostanci2024comet, brasser2017cant, devaux2021method, didio2023copyonflip, enomoto2022efficient, enterprise2015hpmoonshot, fakhrzadehgan2022safeguard, france2022modeling, france2022reducing, frigo2020trrespass, gautam2019rowhammering, gomez2016dram_rowhammer, greenfield2012throttling, guderamarao2023defending, guha2022criticality, han2021surround, hassan2019crow, hassan2021uncovering, hassan2024acase, irazoqui2016mascat, joardar2022learning, joardar2022machine, juffinger2023csirowhammercryptographic, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, kim2023a11v, konoth2018zebram, lee2019twice, lee2021cryoguard, lenovo2015rowhammer, loughlin2021stop, loughlin2022moesiprime, manzhosov2022revisiting, marazzi2023protrr, mutlu2023fundamentally, olgun2024abacus, park2020graphene, park2022rowhammer_reduction, qureshi2022hydra, ryu2017overcoming, saileshwar2022randomized, saroiu2022howto, saroiu2022theprice, saxena2022aqua, saxena2023ptguard, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, sharma2022areview, son2017making, tomita2022extracting, vanderveen2018guardion, vig2018rapid, wang2021discreetpara, wi2023shadow, woo2023scalable, woo2023scalable, yaglikci2021blockhammer, yaglikci2021security, yaglikci2022hira, yang2016suppression, yang2017scanning, you2019mrloc, zhang2020leveraging, zhang2022softtrr, zhou2022ltpim, zhou2023dnndefender}}



\newcommand{\swBasedRowHammerMitigations}[0]{\cite{aweke2016anvil, bock2019riprh, brasser2017cant, enomoto2022efficient, konoth2018zebram, vanderveen2018guardion, zhang2022softtrr}}



\newcommand{\mcBasedRowHammerMitigations}[0]{\cite{aichinger2015ddrmemory, ajorpaz2022evax, apple2015about, arikan2022processor, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, brasser2017cant, devaux2021method, didio2023copyonflip, enomoto2022efficient, enterprise2015hpmoonshot, fakhrzadehgan2022safeguard, france2022modeling, france2022reducing, frigo2020trrespass, gautam2019rowhammering, greenfield2012throttling, guderamarao2023defending, guha2022criticality, han2021surround, hassan2021uncovering, hassan2024acase, irazoqui2016mascat, joardar2022learning, joardar2022machine, juffinger2023csirowhammercryptographic, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, kim2023a11v, konoth2018zebram, lee2019twice, lee2021cryoguard, lenovo2015rowhammer, loughlin2021stop, loughlin2022moesiprime, manzhosov2022revisiting, mutlu2023fundamentally, park2020graphene, park2022rowhammer_reduction, qureshi2022hydra, ryu2017overcoming, saileshwar2022randomized, saroiu2022howto, saroiu2022theprice, saxena2022aqua, saxena2023ptguard, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, sharma2022areview, son2017making, vanderveen2018guardion, vig2018rapid, wi2023shadow, woo2023scalable, yaglikci2021blockhammer, yaglikci2022hira, yang2017scanning, you2019mrloc, zhang2020leveraging, zhang2022softtrr, zhou2022ltpim, zhou2023dnndefender}}



\newcommand{\inDRAMRowHammerMitigations}[0]{\cite{bennett2021panopticon, gomez2016dram_rowhammer, hassan2019crow, hong2023dsac, jedec2017jesd794b, jedec2020jesd794c, marazzi2022rega, marazzi2023protrr, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, yaglikci2021security, yang2016suppression}}





\newcommand{\deterministicRowHammerDefenseCitations}[0]{\cite{bains2016rowhammer, kang2020cattwo, kim2014architectural, kim2022mithril, lee2019twice, park2020graphene, saileshwar2022randomized, saxena2022aqua, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, yaglikci2021blockhammer}}



\newcommand{\probabilisticRowHammerDefenseCitations}[0]{\cite{kim2014flipping, son2017making, you2019mrloc}}



\newcommand{\refreshBasedRowHammerDefenseCitations}[0]{\cite{apple2015about, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, bostanci2024comet, devaux2021method, enterprise2015hpmoonshot, frigo2020trrespass, hassan2021uncovering, irazoqui2016mascat, joardar2022learning, joardar2022machine, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, lee2019twice, lenovo2015rowhammer, loughlin2021stop, marazzi2023protrr, olgun2024abacus, park2020graphene, qureshi2022hydra, saroiu2022howto, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, son2017making, vig2018rapid, wang2021discreetpara, yaglikci2021security, yaglikci2022hira, you2019mrloc, zhang2022softtrr}}



\newcommand{\throttlingBasedRowHammerDefenseCitations}[0]{\cite{greenfield2012throttling, yaglikci2021blockhammer}}



\newcommand{\integrityBasedRowHammerDefenseCitations}[0]{\cite{ajorpaz2022evax, didio2023copyonflip, fakhrzadehgan2022safeguard, guderamarao2023defending, juffinger2023csirowhammercryptographic, manzhosov2022revisiting, saxena2023ptguard}}



\newcommand{\isolationBasedRowHammerDefenseCitations}[0]{\cite{bock2019riprh, brasser2017cant, hassan2019crow, konoth2018zebram, loughlin2021stop, saileshwar2022randomized, saxena2022aqua, vanderveen2018guardion, wi2023shadow, woo2023scalable, woo2023scalable, zhou2023dnndefender}}

\newcommand{\migrationBasedRowHammerDefenseCitations}[0]{\cite{hassan2019crow, saileshwar2022randomized, saxena2022aqua, wi2023shadow, woo2023scalable}}


\newcommand{\circuitBasedRowHammerDefenseCitations}[0]{\cite{gautam2019rowhammering, gomez2016dram_rowhammer, han2021surround, hassan2019crow, hassan2024acase, kim2023a11v, lee2021cryoguard, park2022rowhammer_reduction, ryu2017overcoming, yang2016suppression, yang2017scanning, zhou2022ltpim}}



\newcommand{\detectionOnlyCitations}[0]{\cite{arikan2022processor, france2022reducing, zhang2020leveraging, zhou2022ltpim}}



\newcommand{\surveyCitations}[0]{\cite{aichinger2015ddrmemory, mutlu2023fundamentally, saroiu2022theprice, sharma2022areview}}



\newcommand{\systemImprovementBasedDefenseCitations}[0]{\cite{guha2022criticality, loughlin2021stop, loughlin2022moesiprime}}



\newcommand{\dramStandardCitations}[0]{\cite{jedec2008ddr3, jedec2008jesd79f, jedec2010jesd218, jedec2010jesd219, jedec2012ddr4, jedec2013standard, jedec2014lowpower, jedec2016jesd232a, jedec2020jesd795, jedec2021jesd235d, jedec2021jesd250c, jedec2022high, micron2014sdram, micron2014tn4003}}





\newcommand{\inDRAMRowAddressMappingCitations}[0]{\cite{barenghi2018softwareonly, cojocar2020arewe, horiguchi1997redundancy, itoh2001vlsi, keeth2001dram_circuit, keeth2007dram_circuit, khan2016parbor, khan2017detecting, kim2014flipping, lee2017designinduced, liu2013anexperimental, patel2020bitexact, seshadri2015gatherscatter, smith1981laser, tatar2018defeating}}



\newcommand{\rowHammerGetsWorseCitations}[0]{\cite{cojocar2020arewe, frigo2020trrespass, kim2014flipping, kim2020revisiting, luo2023rowpress, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_a, mutlu2023fundamentally}}



\newcommand{\rowHammerDefenseScalingProblemsCitations}[0]{\cite{hassan2021uncovering, kim2020revisiting, mutlu2017therowhammer, mutlu2018rowhammer, mutlu2019rowhammer_a, mutlu2023fundamentally, park2020graphene}}



\newcommand{\rhdefinition}[0]{\cite{kim2014flipping, kim2020revisiting, mutlu2017therowhammer, mutlu2019rowhammer_a, park2016experiments, park2016statistical, walker2021ondram, yaglikci2022understanding, yang2019trapassisted}}

\newcommand{\rhdefrefresh}[0]{\cite{apple2015about, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, devaux2021method, frigo2020trrespass, hassan2021uncovering, joardar2022learning, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, lee2019twice, lee2021cryoguard, marazzi2023protrr, park2020graphene, qureshi2022hydra, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, son2017making, yaglikci2021security, you2019mrloc, zhang2022softtrr}}

\newcommand{\rhdef}[0]{\cite{apple2015about, aweke2016anvil, bains2015method, bains2016distributed, bains2016rowhammer, brasser2017cant, frigo2020trrespass, greenfield2012throttling, hassan2021uncovering, joardar2022learning, juffinger2023csirowhammercryptographic, kang2020cattwo, kim2014architectural, kim2014flipping, kim2022mithril, konoth2018zebram, lee2019twice, lee2021cryoguard, marazzi2023protrr, park2020graphene, qureshi2022hydra, saileshwar2022randomized, seyedzadeh2017counterbased, seyedzadeh2017mitigating, seyedzadeh2018mitigating, son2017making, vanderveen2018guardion, yaglikci2021blockhammer, yaglikci2021security, you2019mrloc, zhang2022softtrr}}

\newcommand{\perrefreshscaling}[0]{\cite{baumann2005radiationinduced, chang2014improving, kang2014coarchitecting, liu2012raidr, liu2013anexperimental, mukundan2013understanding, nair2013archshield, nair2014refresh, nguyen2018nonblocking}}

\newcommand{\rhsafe}[0]{\cite{frigo2020trrespass, lee2014green, micron2014sdram}}

\newcommand{\rhworse}[0]{\cite{deridder2021smash, frigo2020trrespass, hassan2021uncovering, jattke2022blacksmith, kim2014flipping, kim2020revisiting, mutlu2017therowhammer, mutlu2019rowhammer_a, orosa2021adeeper, yaglikci2022understanding}}

\newcommand{\rhdefworse}[0]{\cite{hassan2021uncovering, kim2020revisiting, orosa2021adeeper, park2020graphene, qureshi2022hydra, yaglikci2021blockhammer, yaglikci2021security}}

\newcommand{\rhattacks}[0]{\cite{aga2017when, bhattacharya2016curious, bosman2016dedup, brasser2017cant, burleson2016invited, cojocar2019exploiting, cojocar2020arewe, deridder2021smash, frigo2018grand, frigo2020trrespass, gruss2015rowhammerjs_a, gruss2018another, hassan2021uncovering, hong2019terminal, jang2017sgxbomb, jattke2022blacksmith, ji2019pinpoint, kim2014flipping, kogler2022halfdouble, kwong2020rambleed, lipp2018nethammer, mutlu2017therowhammer, mutlu2019rowhammer_a, pessl2016drama_exploiting, qiao2016anew, razavi2016flip, safari2014rowhammer, seaborn2015exploiting, tatar2018defeating, tol2022toward, vanderveen2016drammer_deterministic, vanderveen2018guardion, weissman2020jackhammer, xiao2016onebit, yao2020deephammer, zhang2020pthammer}}

\newcommand{\salprefs}[0]{\cite{chang2014improving, kim2012acase, wang2020figaro, zhang2014cream}}

